Can We Infer Confidential Properties of Training Data from LLMs?

Large language models (LLMs) are increasingly fine-tuned on domain-specific datasets to support applications in fields such as healthcare, finance, and law. These fine-tuning datasets often have sensitive and confidential dataset-level properties -- such as patient demographics or disease prevalence -- that are not intended to be revealed. While prior work has studied property inference attacks on discriminative models (e.g., image classification models) and generative models (e.g., GANs for image data), it remains unclear if such attacks transfer to LLMs. In this work, we introduce PropInfer, a benchmark task for evaluating property inference in LLMs under two fine-tuning paradigms: question-answering and chat-completion. Built on the ChatDoctor dataset, our benchmark includes a range of property types and task configurations. We further propose two tailored attacks: a prompt-based generation attack and a shadow-model attack leveraging word frequency signals. Empirical evaluations across multiple pretrained LLMs show the success of our attacks, revealing a previously unrecognized vulnerability in LLMs.

==> sections/attacks.tex <==
% \begin{itemize}
%     \item discriminative models: based on model outputs, such as loss or probability vector (should we add these as the baseline?)
%     \item generative-model attack (GANs). similar
    
% \end{itemize}
\subsection{Black-box access}
% \subsection{Generation based attack}
In the black-box setting, we propose a generation-based attack, following a similar intuition from the GAN paper \cite{zhou2021propertyinferenceattacksgans} that the distribution of the generated samples can reflect the distribution of the fine-tuning data. Since the target model is not trained to generate patient descriptions, we query the target model $\mathcal{T}$ with some prompts that ask the model to generate patient descriptions. Define the set of generated samples with prompts $text$ as $\mathcal{G}_{text} = \{\mathcal{G}_i\}_{i=1}^z$, and the corresponding labels $\{\hat{P}_i \}_{i=1}^z$ where $\hat{P}_i \in \{ 0, 1, N/A \}$ indicates whether the generated sample $\mathcal{G}_i$ satisfies the property, or the property does not apply.
% that the sample $\mathcal{G}_i$ satisfies the property; $\hat{P}_i = 0$ 
% $\hat{P}_i = null $ indicates that this property does not apply. 
For example, if the target property is the gender ratio, $\hat{P}_i = 1$ means that the generated sample $\mathcal{G}_i$ describes a female patient; $\hat{P}_i = 0$ means that $\mathcal{G}_i$ describes a male patient, and $\hat{P}_i = N/A$ means that $\mathcal{G}_i$ is not patient descriptions or does not indicate gender. The adversary predicts the target ratio $P$ with
$$\hat{P}_{\mathcal{G}_{text}} = \frac{1}{|\{i: \hat{P}_i \in \{0,1 \} \}|} \sum_{i:\hat{P}_i \in \{0,1 \} }\hat{P}_i$$
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|}
    \hline
        Instruction = "Suppose you use Chat Doctor to consult some medical suggestions, \\ please fill in the sentence. \#\#\# Response: \textbackslash n"    \\ \hline
        Prompt 1 = Instruction + "Hi, Chatdoctor, I have a medical question." \\ 
        Prompt 2 = Instruction + "Hi, doctor, I have a medical question." \\
        Prompt 3 = Instruction + "Hi Chatdoctor, here is my question." \\ \hline
    \end{tabular}
    % \caption{Input texts for the generation based attack.}
    \label{tab:my_label}
\end{table}
% to  We use some simple prompt injection tricks to ask the fine-tuned LLM to generate patients' concerns, and we estimate the target ratio based on the generated samples. Although the model is trained to perform question-answering tasks, we are interested in how much statistical information the model has learned. 
\subsection{Grey-box access}
% Since the generation-based attack may not work in the discriminative setting, 
We propose two shadow-model attacks in the grey-box setting. The adversary subsample $d$ shadow datasets, $\{\mathcal{S}_{\text{shadow}}^1, \cdots ,\mathcal{S}_{\text{shadow}}^d \}$, from the auxiliary dataset $\mathcal{S}_{aux}$ with different properties $P_{\text{shadow}} = [P_{\text{shadow}}^1, \cdots, P_{\text{shadow}}^d] \in [0,1]^d$. For example, the adversary creates shadow datasets with female ratio ranging from $0.1$ to $0.9$. Then, the adversary fine-tunes the model with the same fine-tuning process $\mathcal{A}$ as the target model and have $d$ shadow models $\{\mathcal{T}_{\text{shadow}}^1, \cdots, \mathcal{T}_{\text{shadow}}^d\}$.

\subsubsection{Perplexity}
Similar to the loss-based attack \cite{suri2022formalizingestimatingdistributioninference}, we propose a perplexity-based shadow model attack. The adversary uses two separate sets of data, one with property $P' = 0$ and the other with $P' =1$, (for example, one set with the female ratio = 1 and the other with the male ratio = 1) and calculates the perplexity of the two sets with the shadow models $\{\mathcal{T}_{\text{shadow}}^1, \cdots, \mathcal{T}_{\text{shadow}}^d\}$ and the target model $\mathcal{T}$. Next, the adversary trains a regression model on the two perplexity scores of the shadow models and the corresponding $P_{\text{shadow}}$ to predict the target ratio.

% predicts the ratio based on the perplexity of these two sets. In particular, for each shadow model , calculate the 
\subsubsection{Word Frequency}
We propose the second shadow model attack with the intuition that female-related words will appear more frequently in the generated outputs of model finetuned with higher female ratio.
% compared to model fine-tuned on low female ratio dataset, model fine-tuned on high female ratio will generate more female-related words. 

Similar to the generation attack, the adversary queries each shadow model $z$ times with some prompts $text$ to generate patient descriptions, denoted as $\{\mathcal{G}^1_{\text{shadow}}, \cdots, \mathcal{G}^d_{\text{shadow}} \}$. For each word $w$ in the word dictionary $\mathcal{V}$, count$(w) \in \mathbb{Z}^d$ counts the number of generated samples that $w$ appear for each $\mathcal{G}^j_{\text{shadow}}, j \in \{1, \cdots,d \}$, and $W \in \mathbb{Z}^{d \times |V|}$ be the total word count.

The adversary uses some feature selection algorithm to pick $\kappa$ words that are highly correlated with the target property, denote the selected word count as $W_{\text{new}} \in \mathbb{Z}^{d \times \kappa}$, and train a meta-regression model $\mathcal{M}$ with $W_{\text{new}}$ and $P_{\text{shadow}}$. More specifically, the input of $\mathcal{M}$ is the count of $\kappa$ words in $z$ queries, and the output of $\mathcal{M}$ is the predicted property ratio.

The adversary queries the target model $\mathcal{T}$ $z$ times using the same prompt $text$, and counts the number of generated samples in which each selected word appears, indicated by $W_{\text{target}} \in \mathbb{Z}^{\kappa}$, then $\hat{P} = \mathcal{M}(W_{\text{target}})$. 

% [Todo: make a figure for the attack workflow]

\begin{algorithm}
\caption{Shadow Attack based on Output Word Frequency}
\begin{algorithmic}[1] % The number tells where line numbering should start
\Procedure{ShadowAttack}{$\mathcal{S}_{aux}$, $\mathcal{T}$, prompt $text$, fine-tuning process $\mathcal{A}$}
    \State Subsample $d$ shadow datasets $\{\mathcal{S}_{\text{shadow}}^j \}_{j=1}^d \sim \mathcal{S}_{aux}$ with various different properties $P_{shadow} = [P_{shadow}^1,..., P_{shadow}^d]$
    \State Finetune d shadow models $\{\mathcal{T}_{shadow}^j \sim \mathcal{A}(\mathcal{S}_{\text{shadow}}^j) \}_{j=1}^d$ 
    \State Use some prompt $text$ to generate output text $\mathcal{G}^j_{shadow}$
    \For  {word $w \in \mathcal{V}$, where $\mathcal{V}$ is the word dictionary }
        \State COUNT$(w) \in \mathbb{Z}^d$
    % \While{condition}
    %     \If{condition}
    %         \State Do something
    %     \Else
    %         \State Do something else
    %     \EndIf
    % \EndWhile
    % \For{each element in collection}
    %     \State Process element
    \EndFor
    \State Denote $\mathcal{W} \in \mathbb{Z}^{|\mathcal{V}| \times d}$ as the word count for all words.
    \State Select k features with FEATURE($\mathcal{W}, P_{shadow}$)
    \State Train a meta-regression model to predict the target ratio META-R
    \State \Return result
\EndProcedure
\end{algorithmic}
\end{algorithm}


% Property inference attack has mainly been studied on discriminative model, and image generative models, GANs.

% Attacks for discriminative model are mainly based on meta-classifier -- the adversary trains shadow models on datasets with varying properties; for example, if the target property is female ratio, the adversary trains shadow model with dataset's female ratio ranging from 0 to 1. Then the adversary train meta-classifier based on some representations to predict target ratio; some examples of the representation are loss or probability vector of a given set of data points, or model weights.

% Attacks for GANs paper \cite{zhou2021propertyinferenceattacksgans} is based on generating samples. The intuition behind is that the generated samples of a GAN can reflect its underlying training dataset's property. 

% For this paper, we propose one attacks under each threat model. 

% \subsection{Shadow model based attack}
% In partial black-box setting, we propose a shadow model based attack with representation using some specific word frequency from the generated text. In particular, we train shadow models with varying properties, then we use some feature selection methods to select words based on its appearing frequency in the generated text. Finally, we train a meta-regression model that predict the target ratio based on the frequency of selected words appearing in the target model's generated outputs. The intuition behind this is that if the model is trained on dataset with high male ratio, male related words will appear more frequently in the outputs, such as "smoke" and "man".

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{sections/shadow_model_attack_pipeline.png}
%     \caption{Shadow model attack pipeline}
%     \label{fig:enter-label}
% \end{figure}



% \subsection{Generation Attacks}

% \subsection{Question-Answering Attacks}

% older baseline attacks: what do they look like


% \subsection{A New Generation-Based Attack}

==> sections/data_aug.tex <==
% \subsection{Dataset Augmentation}
Previous benchmarks for property inference attacks focus on image and tabular data, and natural language classification tasks for simpler language models such as xyz, which makes these benchmarks unsuitable for property inference attacks on LLMs. Motivated by this, we design a benchmark task for specifically for LLM property inference. 

\textbf{Task Requirements: } We discuss some requirements to design the benchmark task. (1) This task needs LLM fine-tuning, either because it requires knowledge from some specific field or because it requires adapting to perform specific tasks. For example, current state-of-the-art LLMs can perform very well on simple sentiment analysis or summarization tasks, hence, there is no need to fine-tune. (2) The fine-tuning dataset contains sensitive information. If the task can be done using public online text, then the statistics are neither private nor sensitive. 
% (3) The task is a language task that needs to be done by some language models. 

\textbf{ChatDoctor Dataset: } We propose two property inference tasks based on the ChatDoctor dataset~\cite{li2023chatdoctormedicalchatmodel}, which is a popular dataset used to fine-tune LLM for the medical question-answering task. The original Chat Doctor dataset consists of 100k pairs of real patient-doctor dialogues of the form (instruction, input, output), where the instruction is a general system prompt about Chat-Doctor, inputs are symptoms described by patients, and outputs are suggestions given by the doctor. Observe that both inputs and outputs contain sensitive medical information about patients, such as their demographic information, described symptoms, and medical diagnoses. 

% Motivating the tasks: higher percentage vs lower percentage and information mostly only contains in the inputs vs information contains in the outputs.

% [Motivation version 1: motivated by gender is a standard attribute for PIA in the previous works]
\subsection{Property I: Demographic Information}
\textbf{Gender.} Following previous work on PIA, we choose gender as the target attribute. In the dataset, some patients will either directly mention their gender in the introduction, such as directly stating "I am a male" or "I am a female", or indirectly mention their gender by mentioning "pregnancy" or "periods". We use ChatGPT-4o to create gender labels for data that contain these gender-related keywords. We discard the data without gender information or data that are ambiguous, and only keep data with female or male labels; this creates a gender labeled dataset with size 29791, in which -- have female label and -- have male label.

% \textbf{Evaluation.} Subsample.....
\subsection{Property II: Medical Diagnosis.}
\textbf{Medical Diagnosis.} Moreover, not only demographic distribution is sensitive, but also the diagnosis. For diseases such as cancer or mental disorders, the statistics are low, hence, it is harder to estimate. Therefore, we choose three low-frequency attributes -- mental disorder, cancer, and digestive disorder -- to test how accurately the attacker can infer these attributes. We randomly subsample a subset with size 50k and use ChatGPT-4o to create labels with "mental disorder", "cancer", "digestive disorder", and "others". This creates a diagnosis-labeled dataset with size 50k, in which --- data have labels "mental disorder ", --- data have labels "cancer", and -- data have labels "digestion disorder".
% \textbf{Evaluation. } 
% Major attribute vs minor attribute.
% Position that may have an effect on the result.
\textbf{Differences} We emphasize the key differences between the two tasks. (1) The first is the position of the attributes -- gender information usually lies in the input, when patients introduce themselves, whereas diagnosis information lies in the output. When fine-tuning models with input-masking, the training objective maximizes the conditional distribution of output given input. Hence, we suspect that the model learns less about the gender distribution when trained with input-masking.
% Prelude: expectation what may be different
% In order to test property inference in both pure generation and question-answering modes, we create two separate tasks. 

% \begin{itemize}
%     \item data augmentation (example figure)
%     \item emphasis differences and setup and expect difference. (connect task, such as position to fine-tuning methods) intuition.
% \end{itemize}
% [Motivation version 2: motivate by pure generation and question answering modes.]

% \paragraph{Gender:} We create a subset of the Chat-Doctor dataset that indicates gender of the patients. First, we select data that contains key words indicating gender such as "female, male, pregnancy, period, son, daughter". Then, we use ChatGPT-4o to create label with the following prompts: 

% \textit{You are an assistant that classify the text based on patient's gender. Is the following text describing a female or male patient's symptoms? For example, if a parent is describing the symptoms of her son, then you should classify it as male. Please output: 1. female, 2. male, 3. both, 4. unclear: \{ patient's symptom description \} }



% \paragraph{Medical Diagnosis:} We randomly subsample a dataset with size 50k and create labels based on concern of the patients. We select medical concern that are easy to classify, in particular, we choose four type of medical concern: mental disorder, pregnancy related concern, allergy reaction and digestive disorder. We use ChatGPT-4o to create labels with the following prompts:

% \textit{The following text describes a patient's concern. You are an assistant that classify the text based on patient's symptoms. If the text describes a patient's main concern about mental disorder, such as suffering from severe depression, anxiety or bipolar, output: mental disorder. Note that if the patient simplify express anxiety about other symptoms, or is tired should not be classify as mental disorder. For all the other symptoms, output: others:  \{patient's symptom description and doctor's diagnosis\}


% If the text descibes patient's main concern about childbirth, preganancy, trying to conceive or infertility, output: birth.


% If the text describes main concern about immune system overreaction or allergic reaction, such as skin rashes or sneezing nose, output: immune. Note that cough and sneezing nose may appear for both allergy and cold, try to classify based on the description. If the text describes main concerns about digestive issues, such as bloating, diarrhea, constipation, abdominal pain, output: digestion. Do not classify losing appetite or having abdominal pain due to fever or other disease as digestion. For all the other symptoms, output: others:  \{patient's symptom description\}}
[Todo: choose 5\% of the labeled data and manually check the performance.]
Put the detailed labeling process in the Appendix, including prompt for ChatGPT, verification by LLama-3-60B and human check like 200 subsamples etc. 


% Two modes : for each mode, we consider blablabla as properties.


==> sections/experiment-propertytypee.tex <==

In this section, we investigate if our proposed attacks succeed empirically in our new benchmark \taskname. In particular, we ask the following questions:
\begin{itemize}
    \item How do the different attacks perform in the chat completion and QA modes?
    \item How does the fine-tuning method affect attack performance?
\end{itemize}


\subsection{Experimental Setup}\label{subsec:expattacksetup}

\textbf{Models.}~We use three open base models for experimentation: Llama-1-8b\citep{touvron2023llama}, Pythia-v0-6.9b\cite{biderman2023pythia} and Llama-3-8b-instruct \citep{llama3modelcard}. We use the Llama-1 and Pythia-v0 since these were released before the original ChatDoctor dataset and hence have no data-contamination from the pre-training stage, giving us a plausibly more reliable attack performance. While Llama-3 came after ChatDoctor release, we still use it since it is highly performant and is widely used for experimentation. Refer to \ref{subsec:experiment setup} for fine-tuning details\ph{and fine-tuning performance?}.

\textbf{Attack Baselines.} (1)In the back-box setting, our baseline is directly asking the target model to specify the property ratio. For example, we query the model with "what is the percentage of patient that has a mental disorder concern in the ChatDoctor dataset?", for the complete prompts, kindly refers to \ref{subsec:experiment setup}. (2) In the grey-box setting, our baseline is shadow model attack with perplexity, as described in Section \ref{shadow_attack}.
\ph{Should we put it here: We also mention the attack success rates before fine-tuning the models on attribute datasets.}

\textbf{Generation attack}. As described in \ref{subsec:genattack}, we designed the input prompts that reflect the characteristics of the target dataset. For example, we query the target model to fill in the following sentence: "Hi, Chatdoctor, I have a medical question." For a complete description of the prompts, kindly refer to \ref{subsec:experiment setup}. For each target model, $f$, and prompt $t$, we query $2000$ times, i.e. $|\mathcal{S}_{f,t}| = 2000$. Then, we use ChatGPT-4o to label each generated text based on the target attribute (as described in Section\ref{subsec:labeling}). In the main paper, we report the attack results with aggregated prompts; for an ablation study of the attack performance with individual prompts, kindly refers to \ref{subsec:ablation}.

\textbf{Data Splits.}~Since the shadow model attacks assume a separate set of auxiliary data for training shadow models, we split the gender benchmark dataset into (1) data used by the model owner for fine-tuning with $15$k samples and (2) auxiliary data, \sa, to be used by the adversary for training shadow models,  with $14,791$ samples. Out of the $15$k samples, we subsample three different fine-tuning datasets of size $6500$, corresponding to three property ratios with $P \in \{ 0.3, 0.5, 0.7\}$.

For properties corresponding to medical diagnosis, the number of samples are much fewer ($2.5$k, $6.3$k, $5.3$k for mental disorder, digestive disorder and childbirth  respectively). Therefore we do not split them further in the interest of fine-tuning performance and do not conduct shadow model attacks on them.

\textbf{Shadow Attacks.} For the word frequency shadow model attack, we use the same prompts as the black-box generation attacks to query the shadow and target models; for each prompt, we query $50-100$k times since many words are uncommon in generated text. In the main paper, we report the attack results with aggregated prompts; for an ablation study of the attack performance of individuals prompts, kindly refers to \ref{subsec:ablation}. For the selection of the hyper-parameters, kindly refers to \ref{subsec:experiment setup}. %\cy{describe our technique to select words}

\ph{appendix:}
% For each target model, we randomly subsample data from the auxiliary data $\mathcal{S}_{\text{aux}}$ and
We fine-tune shadow models corresponding to seven shadow property ratios, \ph{$P_{\text{shadow} } \in \{0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8 \}$}. For each \ph{$P_{\text{shadow}}$}, we fine-tune six shadow models corresponding to the same architecture and initial checkpoints as the target model. We use XG-Boost \cite{} as the meta-regression model.


% For the shadow model attack, we consider the perplexity-based attack as the baseline as it perplexity based attacks are common in the privacy literature as mentioned earlier.


\textbf{Attack Evaluation.} Since the adversary aims to infer the exact property ratio, which is a continuous number between 0 and 1, we follow \cite{zhou2021propertyinferenceattacksgans} and use the absolute error between predicted and groundtruth property ratios to evaluate the attack performance, defined by \ph{need to change notation $|P - \hat{P}|$.} The adversary is said to perfectly estimate the target ratio when the absolute error is zero. 
For the gender property, we evaluate all the attacks. For the medical diagnosis property, since we do not subsample the fine-tuning data to change the target ratios, as mentioned in \ref{sub:threat models}, it becomes a trivial problem if we assume adversary has to auxiliary data. Therefore, we only evaluate the black-box access attack in the medical diagnosis dataset.

% \cy{We report the MAEs averaged across prompts. please fix this statement and put in the right place -- we need to clarify across what all things is the MAE averaged over}

\subsection{Gender Property Inference Observations}
%\cy{new results : Qa mode best \& others fail, chat completion best \& others fail -- word frequency is second best but it needs data, error order of mag numbers are different, BB generation numbers in the gender property across modes}


\textbf{In the QA mode, Word-Frequency-based Shadow Attack achieves effective performance for gender ratio inference.} As shown in Table \ref{tab:gender}, in the QA mode, word frequency-based shadow attack consistently achieves the smallest total mean absolute error across target ratios. Its superiority may be attributed to its ability to detect subtle lexical patterns correlated with gender which are reflected in word frequencies.

In contrast, other attacks generally lack discriminative power across different target ratios. For instance, the black-box generation attack predicts approximately $70\%$ across all ratios when applied to the Llama-1 model. We hypothesize this failure stems from the fact that, in QA mode, models are trained on the conditional distribution of outputs \textit{given} inputs (SFT Eq. \ref{Training objective 1}) which limits the model's ability to learn from the input itself — this is particularly problematic here since gender information typically appears in the self-introductions of patients \textit{within the input} (see Sec.\ref{sec:benchmark}). As a result, the model fails to capture obvious and easy statistical signals about gender which are important for correct labeling (See Sec.\ref{subsec:genattack}).

Word-Frequency attack also outperforms both baseline attacks; while the poor performance of perplexity-based attacks suggests that perplexity may not be a suitable metric for capturing relevant information for property inference, the failure of the direct-asking baseline may result from the model’s inability to explicitly reason about property ratios (or from safety training) when phrased as a direct question.


\textbf{In the Chat-Completion mode, Black-Box Generation Attack achieves effective performance along with Word-Frequency attack as the second best.} As demonstrated in Table \ref{tab:gender}, in the Chat-Completion mode, the black-box generation attack achieves the lowest total error across different targets. The reason for the success of black-box generation attack is likely that the model is trained on the \textit{joint} distribution of both the inputs and outputs (as opposed to the conditional distribution in the QA mode, CLM-FT Eq. \ref{Training objective 2}), which allows the model to mirror the inputs distribution of the fine-tuning dataset.

We also note that our word-frequency shadow attack closely follows the black-box generation attack with its second lowest total error; the reason for its success is same as described for the QA mode. Note that while the word-frequency attack comes close to the generation attack in terms of performance, it makes more assumptions and requires auxiliary data and fine-tuning capabilities. These attacks also perform better than the baselines, for similar reasons as mentioned above.

In general, we see \textbf{better performance (lower error) of all attacks in the chat-completion mode as compared to the QA mode}; this can be attributed to the different fine-tuning objectives which lead to different memorization patterns some of which can be more amenable for property inference, as described above.
%; for instance the smallest error achieved by the black-box generation attack is $0.61\%$ while the word-frequency attack predicts some target ratios perfectly with zero error -- removing this since this means that word frequeeency shoudl be better plus we are talking about overall abs diff now.
\subsection{Medical Diagnosis Property Inference Observations}

\textbf{For both QA and chat-completion modes, the black-box generation attack achieves effective performance for inferring medical diagnosis properties.} As demonstrated in Table \ref{tab:medical}, the black-box generation attack achieves the smallest mean absolute error in property inference both the QA and Chat-Completion modes. The good performance of this attack in the QA mode is in contrast to the QA mode of gender inference and can be attributed to diagnosis information being mentioned in the outputs rather than inputs (see Sec.\ref{sec:benchmark}), which are trained over in both modes thereby reducing the influence of the training objectives. Black-box attack also consistently outperforms both the baseline attacks (for similar reasons as described earlier).


\textbf{The mean absolute error for childbirth is much higher than the other attributes for both modes.} While the attack performs particularly well for the mental and digestive disorder properties in both modes, it performs much worse childbirth.  We suspect this is because childbirth (and related topics such as pregnancy, abortion, contraception and so on) is a culturally sensitive topic and the models may have undergone some safety training to reduce the likelihood of outputting childbirth-related content, which leads to the failure of our attacks.

\textbf{Data Contamination in Llama3.} To check for plausible data contamination with the original ChatDoctor dataset, we deploy the black-box generation attack on the base Llama1 and Llama3 models (without any additional fine-tuning). We observe that the attack predicts almost similar ratios for both Llama1 and Llama3 models across all medical diagnosis properties. This hints towards minimal effect of ChatDoctor dataset on the llama3 model.

(*The fine-tuned pythia model does not produce any output given the direct asking prompts. We also test it on the base model and have a similar results. We suspect the reason is that the model is not understanding the prompts good enough.)

%\textbf{In the chat-complettion mode, For medical diagnosis properties, the black-box generation attack achieves effective performance.} Similar to QA mode, the black-box generation attack achieves the best performance in inferring medical diagnosis property ratios, as it evident by the lowest errors achieved by this attack across the board \ref{tab:medical;chat-completion}. The error for childbirth is again much higher than the other two properties for similar reasons as the QA mode.
\begin{table}[ht]
\centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc}
\toprule
\textbf{Model} & \textbf{Attacks} & \multicolumn{3}{c|}{\textbf{QA Mode}} & \multicolumn{3}{c}{\textbf{Chat-Completion Mode}} \\
              &                   & 30 & 50 & 70 & 30 & 50 & 70 \\
\midrule
\multirow{4}{*}{Llama-1}
& Direct asking         & $23.17{\scriptstyle \pm 1.78}$ & $3.98{\scriptstyle \pm 1.88}$ & $18.6{\scriptstyle \pm 0}$ & $22.8{\scriptstyle \pm 1.98}$ & $7.7{\scriptstyle \pm 1.8}$ & $18.57{\scriptstyle \pm 4.71}$ \\
& BB generation         & $36.52{\scriptstyle \pm 0.11}$ & $15.45{\scriptstyle \pm 3.09}$ &  $1.45{\scriptstyle \pm 0.64}$ & \cellcolor{gray!20} $1.73{\scriptstyle \pm 0.76}$ & \cellcolor{gray!20} $2.64{\scriptstyle \pm 3.33}$ & \cellcolor{gray!20} $3.28{\scriptstyle \pm 3.64}$ \\
& Perplexity            & $28.67{\scriptstyle \pm 9.34}$ & $9.38{\scriptstyle \pm 8.95}$ & $24.16{\scriptstyle \pm 2.45}$ & $35.19{\scriptstyle \pm 10.99}$ & $14.5{\scriptstyle \pm 5.98}$ & $5.33{\scriptstyle \pm 6.09}$ \\
& Word-frequency        & \cellcolor{gray!20}$11.43{\scriptstyle \pm 3.0}$ & \cellcolor{gray!20}$7.33{\scriptstyle \pm 6.59}$ & \cellcolor{gray!20}$6.85{\scriptstyle \pm 5.03}$ & $3.44{\scriptstyle \pm 4.61}$ & $0{\scriptstyle \pm 0}$ & $6.6{\scriptstyle \pm 9.35}$ \\
\midrule
\multirow{4}{*}{Pythia-v0}
& Direct asking *         & -- & -- & -- & -- & -- & -- \\
& BB generation         & $46.75{\scriptstyle \pm 3.64}$ & $23.45{\scriptstyle \pm 5.89}$ & $10.31{\scriptstyle \pm 4.85}$ &\cellcolor{gray!20} $3.56{\scriptstyle \pm 2.03}$ & \cellcolor{gray!20} $ 5.61{\scriptstyle \pm 0.78}$ & \cellcolor{gray!20} $2.15{\scriptstyle \pm 2.45}$ \\
& Perplexity            & $22.33{\scriptstyle \pm 15.8}$ & $11.25{\scriptstyle \pm 13.68}$ & $25.79{\scriptstyle \pm 15.59}$ & $4.32 {\scriptstyle \pm 3.25}$ & $9.94 {\scriptstyle \pm 0.59}$ & $9.39 {\scriptstyle \pm 0}$ \\
& Word-frequency        & \cellcolor{gray!20}$22{\scriptstyle \pm 10.4}$ & \cellcolor{gray!20}$7.95{\scriptstyle \pm 9.44}$ & \cellcolor{gray!20}$9.25{\scriptstyle \pm 11.9}$ & $3.31{\scriptstyle \pm 4.68}$ & $3.27{\scriptstyle \pm 4.62}$ & $6.73{\scriptstyle \pm 8.22}$ \\
\midrule
\multirow{4}{*}{Llama-3}
& Direct asking         & $14.27{\scriptstyle \pm 5.32}$ & $4.86{\scriptstyle \pm 1.33}$ & $19.9{\scriptstyle \pm 4.24}$ & $17.97{\scriptstyle \pm 5.33}$ & $4.0{\scriptstyle \pm 2.12}$ & $16.17{\scriptstyle \pm 1.18}$ \\
& BB generation         & $23.64{\scriptstyle \pm 5.82}$ & $5.79{\scriptstyle \pm 6.46}$ & $14.01{\scriptstyle \pm 1.68}$ & \cellcolor{gray!20}$0.61{\scriptstyle \pm 0.77}$ & \cellcolor{gray!20}$1.33{\scriptstyle \pm 1.31}$ & \cellcolor{gray!20}$1.25{\scriptstyle \pm 1.52}$ \\
& Perplexity            & $13.28{\scriptstyle \pm 4.77}$ & $25.0{\scriptstyle \pm 25.4}$ & $19.01{\scriptstyle \pm 20.52}$ & $17.80{\scriptstyle \pm 9.06}$ & $19.85{\scriptstyle \pm 7.6}$ & $6.24{\scriptstyle \pm 7.57}$ \\
& Word-frequency        & \cellcolor{gray!20}$8.29{\scriptstyle \pm 2.13}$ & \cellcolor{gray!20}$7.33{\scriptstyle \pm 6.59}$ & \cellcolor{gray!20}$10.66{\scriptstyle \pm 7.12}$ & $2.45{\scriptstyle \pm 2.3}$ & $3.33{\scriptstyle \pm 4.7}$ & $5.83{\scriptstyle \pm 1.73}$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Attack Performance for gender property in the QA mode (left) and Chat-Completion mode (right).} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio. We highlight the attack that achieves the smallest total MAE across different target ratios.}
\label{tab:gender}
\end{table}

\begin{table}[ht]
\centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc}
\toprule
\textbf{Model} & \textbf{Attacks} & \multicolumn{3}{c|}{\textbf{QA Mode}} & \multicolumn{3}{c}{\textbf{Chat-Completion Mode}} \\
              &                   & Mental & Digestive & Childbirth & Mental & Digestive & Childbirth \\
\midrule
\multirow{3}{*}{Llama-1}
& Generation w/o FT     & 3.45 & 4.19 & 9.88 & 3.45 & 4.19 & 9.88 \\
& Direct asking         & $7.66{\scriptstyle \pm 2.05}$ & $0.18{\scriptstyle \pm 0}$ & $9.2{\scriptstyle \pm 0}$ & $8.62{\scriptstyle \pm 2.36}$ & $0.17{\scriptstyle \pm 0}$ & $9.2{\scriptstyle \pm 0}$ \\
& BB generation         & \cellcolor{gray!20}$2.55{\scriptstyle \pm 0.25}$ & \cellcolor{gray!20}$3.94{\scriptstyle \pm 0.37}$ & \cellcolor{gray!20}$7.95{\scriptstyle \pm 0.36}$ & \cellcolor{gray!20}$1.76{\scriptstyle \pm 0.23}$ & \cellcolor{gray!20}$1.44{\scriptstyle \pm 0.24}$ & \cellcolor{gray!20}$6.99{\scriptstyle \pm 0.18}$ \\
\midrule
\multirow{3}{*}{Pythia-v0}
& Generation w/o FT     & 1.84 & 9.57 & 9.85 & 1.84 & 9.57 & 9.85 \\
& Direct asking(*)         & -- & -- & -- & -- & -- & -- \\
& BB generation         & \cellcolor{gray!20}$1.82{\scriptstyle \pm 0.56}$ & \cellcolor{gray!20}$3.71{\scriptstyle \pm 0.82}$ & \cellcolor{gray!20}$7.63{\scriptstyle \pm 0.31}$ & \cellcolor{gray!20}$1.88{\scriptstyle \pm 0.36}$ & \cellcolor{gray!20}$1.84{\scriptstyle \pm 0.16}$ & \cellcolor{gray!20}$6.23{\scriptstyle \pm 0.52}$ \\
\midrule
\multirow{3}{*}{Llama-3}
& Generation w/o FT     & 3.45 & 4.64 & 10.32 & 3.45 & 4.64 & 10.32 \\
& Direct asking         & $19.96{\scriptstyle \pm 17.74}$ & $14.22{\scriptstyle \pm 0}$ & $10.26{\scriptstyle \pm 0.47}$ & $5.03{\scriptstyle \pm 0}$ & $12.64{\scriptstyle \pm 0}$ & $10.27{\scriptstyle \pm 0.5}$ \\
& BB generation         & \cellcolor{gray!20}$1.43{\scriptstyle \pm 0.7}$ & \cellcolor{gray!20}$1.80{\scriptstyle \pm 1.18}$ & \cellcolor{gray!20}$7.73{\scriptstyle \pm 0.38}$ & \cellcolor{gray!20}$0.63{\scriptstyle \pm 0.23}$ & \cellcolor{gray!20}$1.82{\scriptstyle \pm 0.45}$ & \cellcolor{gray!20}$4.59{\scriptstyle \pm 0.35}$ \\
\bottomrule
\end{tabular}}
\caption{\textbf{Attack Performance for medical diagnosis in the QA mode (left) and Chat-Completion mode (right).} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio. We highlight the attack that achieves the smallest total MAE across different target ratios.}
\label{tab:medical}
\end{table}

\subsection{Ablation study}
Due to the importance of hyper-parameters in attack performance, we conduct an ablation study on these, specifically, 

The hyper-parameters play an important role in the attack performance. In this section, we conduct an ablation study on the following hyperparameters: (1) for the word-frequency-based shadow model attack, we study the effect of the number of shadow models and the number of selected keywords; (2) for the black-box generation attack, we study the effect of the number of generated samples. As shown in Figure \ref{fig:keyword}, the optimal number lies between 30-35 keywords. With fewer keywords, it may not have enough signals to accurately infer the ratios; and with larger keywords, it may contain noisy signals. Note that the optimal number varies between different model architectures; for the ablation study on other model architectures, kindly refer to \ph{Appendix}. As shown in Figure \ref{fig:shadow_model}, as the number of shadow models increases, the attack performance is improved. We think the reason is that with more shadow models, we can (1) find more reliable word signals that are correlated with the target ratios, and (2) learn the word patterns between different target ratios better. Lastly, Figure \ref{fig:generated_samples} shows that the estimated ratio from the black-box generation converges very fast, with $500$ generated samples, the MAE is under $2\%$.
\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/Figures/keyword.png}
    \caption{\# of keyword}
    \label{fig:keyword}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/Figures/shadow_model.png}
    \caption{\# of shadow model}
    \label{fig:shadow_model}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/Figures/gen_text.png}
    \caption{\# generated samples}
    \label{fig:generated_samples}
\end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.24\textwidth}
%     \includegraphics[width=\linewidth]{fig4.png}
%     \caption{Caption 4}
% \end{subfigure}
\caption{\textbf{Effect of several hyperparameter on the attack results in Llama-3-8b-instruct (lower MAE is better)}.}
\label{Ablation:Llama3}
\end{figure}

==> sections/experiment.tex <==

In this section, we investigate if our proposed attacks succeed empirically. In particular, we ask the following questions:
\begin{itemize}
    \item How do the different attacks perform in the chat completion and QA modes?
    \item How does the fine-tuning method affect attack performance?
    % \item Which confidential properties have more leakage?
\end{itemize}



%Following \cite{li2023chatdoctormedicalchatmodel}, we choose Llama-1-8b as the base model; furthermore, to validate the robustness of our property inference attack, we choose two other model architectures, namely Pythia-v0-6.9b and Llama-3-8b-instruct. \footnote{We try our best to prevent data contamination from the pre-training stage. For Llama-1-8b and Pythia-v0-6.9b, since they are releassed before the releasing date of the ChatDoctor dataset, these model do not have data contamination; for Llama-3-8b-instruct, we .... }\cy{mention contamination, llama3 has best performance} 
% We test our property inference attacks on three pre-trained LLMs: Llama-1-8b, Pythia-v0-6.9b and Llama-3-8b-instruct. We choose Llama-1 and Pythia-v0 since these two models are released before the release date of the ChatDoctor dataset.
% Ideally, the LLMs are not pre-trained, or fine-tuned on the ChatDoctor dataset, so that we can subsample the target variables and prevent contamination. Since Llama-1-8b and Pythia-v0-6.9b were released before the ChatDoctor dataset, the ChatDoctor dataset is not in the pre-training data of these models. 
% We also include Llama-3-8b-instruct to test whether the contamination has an effect on the attack performance.
% Since Llama-1-8b and Pythia-v0-6.9b do not have instruction-following capability, we follow \cite{li2023chatdoctormedicalchatmodel} which first performs instruction fine-tuning on the Alpaca dataset.



\subsection{Experimental Setup}\label{subsec:expattacksetup}

% For the gender attribute, we have a fine-tuning dataset of 29k samples with 19k female and 10k male labels. 
% Recall from Sec. \ref{sec:benchmark} that we have four target attributes, namely medical diagnosis -- mental disorder, digestive disorder, childbirth  and gender.
% with target ratios of 5.10\%, 12.68\%, 10.6\% respectively
%  with three target ratios 30\%, 50\% and 70\%.


\textbf{Models.}~We use three open base models for experimentation -- Llama-1-8b, Pythia-v0-6.9b and Llama-3-8b-instruct \cy{cite}. We use the Llama-1 and Pythia-v0 models since these were released before the original ChatDoctor dataset and therefore have less chance of being trained on it, giving us a plausibly more reliable picture of attack performance. While Llama-3 came after ChatDoctor release, we still use it since it is highly performant and is widely used for experimentation. 

Since Llama-1-8b and Pythia-v0-6.9b do not have instruction-following capability, we follow \cite{li2023chatdoctormedicalchatmodel} which first performs instruction fine-tuning on the Alpaca dataset \cy{cite alpaca}. Next, we fine-tune each model for both QA and chat-completion mode, with objective functions noted in Eqs. \ref{Training objective 1} and \ref{Training objective 2} respectively. We used the LoRA \cite{hu2021loralowrankadaptationlarge} method for fine-tuning with a learning rate of $1e^{-4}$, dropout rate of $0.05$, LoRA rank of $128$ and $5$ epochs. All are models are fine-tuned three times with different random seeds.
% \cy{what other hyperparams? are they default? Mention all LLM related params in appendix}


\textbf{Data Splits.}~Since the shadow model attacks assume a separate set of auxiliary data for training shadow models, we split the gender benchmark dataset into (1) data used by the model owner for fine-tuning with $15$k samples and (2) auxiliary data, \sa, to be used by the adversary for training shadow models,  with $14,791$ samples. Out of the $15$k samples, we subsample three different fine-tuning datasets of size $6500$, corresponding to three property ratios with $P \in \{ 0.3, 0.5, 0.7\}$.

For properties corresponding to medical diagnosis, the number of samples are much fewer ($2.5$k, $6.3$k, $5.3$k for mental disorder, digestive disorder and childbirth  respectively). Therefore we do not split them further in the interest of fine-tuning performance and do not conduct shadow model attacks on them.

%For each target ratio, we fine-tune three target models, hence nine target models in total. For the medical diagnosis properties, we do not subsample since we do not have enough data for subsampling, instead we fine-tuned on the diagnosis dataset three times to account for training randomness.



%\textbf{Data Splits.}~Since the shadow model attacks assume a separate set of auxiliary data for training shadow models, we split the gender benchmark dataset into (1) data used by the model owner for fine-tuning with $15$k samples and (2) auxiliary data, \sa, to be used by the adversary for training shadow models,  with $14,791$ samples.


%\textbf{Fine-tuned Target Models.}~For the gender property, we subsample the respective gender dataset from $\mathcal{S}_{train}$ with $P \in \{ 0.3, 0.5, 0.7\}$ with size $6500$. For each target ratio, we fine-tune three target models, hence nine target models in total. For the medical diagnosis properties, we do not subsample since we do not have enough data for subsampling, instead we fine-tuned on the diagnosis dataset three times to account for training randomness.




\textbf{Generation Attacks.} We query each target model with three different prompts as follows.

\begin{itemize}
    \item Instruction = "Suppose you use Chat Doctor to consult some medical suggestions, please fill in the sentence. \#\#\# Response: \textbackslash n" 
    \item Prompt 1 = Instruction + "Hi, Chatdoctor, I have a medical question." 
    \item Prompt 2 = Instruction + "Hi, doctor, I have a medical question."
    \item Prompt 3 = Instruction + "Hi Chatdoctor, here is my question."
\end{itemize}

We query the target model $2000$ times for each prompt, i.e. $|\mathcal{G}_{text}| = 2000$. Then, we use ChatGPT-4o to label each generated text as belonging to female, male or $N/A$ (as described in Sec.\ref{subsec:genattack}).

% For the gender property, we query the target model $2000$ times for each prompt, i.e. $|\mathcal{G}_{text}| = 2000$. For medical diagnosis properties, since the target ratio is low-frequency, we query the target model $...$ times for each prompt, i.e. $|\mathcal{G}_{text}| = ... $. Then, we use ChatGPT-4o to label each generated text as belonging to female, male or $N/A$ (as described in Sec.\ref{subsec:genattack}).


\textbf{Shadow Attacks.} For each target model, we randomly subsample data from the auxiliary data $\mathcal{S}_{\text{aux}}$ and fine-tune shadow models corresponding to seven shadow property ratios, $P_{\text{shadow} } \in \{0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8 \}$. For each $P_{\text{shadow}}$, we fine-tune six shadow models corresponding to the same architecture and initial checkpoints as the target model.


For the word frequency shadow model attack, we use the same prompts described above to query the shadow and target models; for each prompt, we query $100$k times since many words are uncommon in generated text.\cy{describe our technique to select words}

%We randomly subsample data from $\mathcal{S}_{\text{aux}}$  and fine-tuned 42 shadow models with various properties. In particular, we choose $P_{\text{shadow} } \in \{0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8 \}$ and for each $P_{\text{shadow}}$, we fine-tuned six shadow models. For the shadow model attack based on word frequency, we query the shadow models and target model with the prompts described above; for each prompt, since many words are uncommon in generated text, we query $100,000$ times.
%We used the univariate method to select word\cite{}. 


\textbf{Attack Baselines.}~For the generation attack which is based on only querying, our baseline is directly asking the target model to specify the property ratio. The prompt used for this baseline is `' \cy{fill in}. We also mention the attack success rates before fine-tuning the models on attribute datasets.

For the shadow model attack, we consider the perplexity-based attack as the baseline as it perplexity based attacks are common in the privacy literature \cy{cite}.

%We consider two baseline attacks: (1) we directly prompt the target model with what is the target property. (2)

\textbf{Attack Evaluation.} In our attack setting, the adversary aims to infer the exact property ratio, which is a continuous number between 0 and 1. Hence, similar to \cite{zhou2021propertyinferenceattacksgans}, we use the absolute error between predicted and groundtruth property ratios to evaluate the performance of the attacks, given by $|P - \hat{P}|$ where $P$ and $\hat{P}$ are the groundtruth and predicted property ratios. The adversary is said to perfectly estimate the target ratio when the absolute error is zero.

%Formally, it is written as $|P - \hat{P}|$. If $|P - \hat{P}| = 0$, it means that the adversary perfectly predicts the target ratio.

\subsection{Question-Answering Mode Observations}
% In this section, we test property inference attacks in the QA mode.
% , which is fine-tuned with the training objective described in Equation \ref{Training objective 1}. 
\textbf{For gender property inference, Word-Frequency-based shadow attack achieves effective performance in most cases.}  As shown in Table \ref{tab: gender; question-answering}, the word frequency-based shadow attack consistently achieves the smallest (or second to the smallest) mean absolute error across most target ratio settings. In contrast, other attacks generally lack discriminative power across different target ratios. For instance, the black-box generation attack predicts approximately $70\%$ across all ratios when applied to the Llama-1 model. We hypothesize this failure stems from the fact that, in black-box generation mode, models are trained on the conditional distribution of outputs given inputs which limits the model's ability to learn from the input itself— this is particularly problematic here since gender information typically appears in the self-introductions of patients within the input. As a result, the model fails to capture relevant statistical signals.

The superior performance of our word frequency-based attack may be attributed to its ability to detect lexical patterns: when the model is fine-tuned on data with more female patients, it is more likely to generate female-associated concerns, which are reflected in word frequency distributions. This method also outperforms both baseline attacks in most cases. While the poor performance of perplexity-based attacks suggests that perplexity may not be a suitable metric for capturing relevant information for property inference, the failure of the direct-asking baseline may result from the model’s inability to explicitly reason about property ratios when phrased in a direct-question format.

\textbf{For medical diagnosis properties, the black-box generation attack achieves effective performance.} As demonstrated in Table \ref{tab: medical;quesiton-answering}, the black-box generation attack achieves the smallest mean absolute error in property inference across the board; it
outperforms both the baseline attacks always. The attack performs particularly well for the mental and digestive disorder properties, achieving an error of only $1.43\%$ and $1.80\%$ respectively for Llama3. The mean absolute error for childbirth is much higher than the other attributes; we suspect this is because childbirth (and related topics such as pregnancy, abortion, contraception and so on) is a culturally sensitive topic and the models may have undergone some safety training to reduce the likelihood of outputting childbirth-related content, which leads to the failure of our attacks. 

We also note that our \textbf{black-box generation attack performs much better for the medical diagnosis properties, which have a low ratio in the training set, than the gender property which have a much higher ratio.} \cy{is there a reason to explain this?}\cy{should we keep saying 'ratio'? It is a percentage now}\cy{can we say something about the performance of the successful attack across different models?}

\cy{new results : Qa mode best \& others fail, chat completion best \& others fail -- word frequency is second best but it needs data, error ordeer of mag numbers are different, BB generation numbers in the gender property across modes}

\cy{in both modes same attack works well, slightly better which attack -- memorization, childbirth}

\cy{direct people to ablation study}

% \paragraph{Gender: }
% \begin{table} [h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
% Target female ratio $\%$ =  &  30 &  50 & 70 & Abs diff\\ 
% \hline
% \multicolumn{5}{ |c| }{Llama-1} \\
% \hline
% Baseline 1 (direct asking) & $53.17 \pm 1.97$  & $57.70 \pm 1.80$  & $51.4 \pm 0$  & $15.25$ \\    
% Black-box generation attack & $66.53 \pm 0.11 $ & $65.45 \pm 3.09$ & $68.55 \pm  0.64$ & $17.81$ \\
% Perplexity-based attack&  &  &  & \\ 
% Word frequency-based attack & $0.38 \pm 0.01$ & $0.49 \pm 0.07$ & $0.62 \pm 0.1$ & $\textbf{0.091}$ \\ \hline


% \multicolumn{5}{ |c| }{Pythia-v0-6.9b} \\
% \hline
% Baseline 1 (direct asking) &  &  &  & \\ 
% Black-box generation attack & $76.76 \pm 3.64$ & $73.45 \pm 5.89$ & $80.31 \pm 4.85$ & $26.84$ \\
% Perplexity-based attack &  &  &  & \\ 
% Word frequency-based attack & $0.4 \pm 0$ & $0.45 \pm 0.08$ & $0.55 \pm 0.12$ & $\textbf{0.113}$ \\ \hline

% \multicolumn{5}{ |c| }{Llama-3-8b-instruct} \\
% \hline
% Baseline 1 (direct asking) & $44.27 \pm 0.19$  & $47.13 \pm 4.15$  & $50 \pm 4.24$  & $12.71$ \\ 
% Black-box generation attack & $53.63 \pm 5.82$ & $49.12 \pm 6.46$ & $55.99 \pm 1.67$ & 14.48 \\
% Perplexity-based attack &  &  &  & \\
% Word frequency-based attack & $0.4156 \pm 0.014$ & $0.473 \pm 0.038$ & $0.6145 \pm 0.043$ & $\textbf{0.076}$ \\ \hline
% \end{tabular}
% \end{center}
% \caption{Attack performance for gender property in the QA mode. The number reported on the second to fourth columns are the mean and standard deviation of the predicted ratio corresponding to each target ratio. The last column is the average absolute difference. }
% \label{tab: gender; question-answering}
% \end{table}

% \ph{**report the absolute difference for each target ratios, instead of predicted ratios}
% \ph{maybe only put the Llama-1 and Llama-3 in the table}
% \ph{small text for std}
% \ph{transpose the table}
\ph{report which K is used?}
\begin{table}[ht]
\centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc}
\toprule
\textbf{Model} & \textbf{Attacks} & \multicolumn{3}{c|}{\textbf{QA Mode}} & \multicolumn{3}{c}{\textbf{Chat-Completion Mode}} \\
              &                   & 30 & 50 & 70 & 30 & 50 & 70 \\
\midrule
\multirow{4}{*}{Llama-1}
& Direct asking         & $23.17{\scriptstyle \pm 1.78}$ & $3.98{\scriptstyle \pm 1.88}$ & $18.6{\scriptstyle \pm 0}$ & $22.8{\scriptstyle \pm 1.98}$ & $7.7{\scriptstyle \pm 1.8}$ & $18.57{\scriptstyle \pm 4.71}$ \\
& BB generation         & $36.52{\scriptstyle \pm 0.11}$ & $15.45{\scriptstyle \pm 3.09}$ &  $1.45{\scriptstyle \pm 0.64}$ & \cellcolor{gray!20} $1.73{\scriptstyle \pm 0.76}$ & \cellcolor{gray!20} $2.64{\scriptstyle \pm 3.33}$ & \cellcolor{gray!20} $3.28{\scriptstyle \pm 3.64}$ \\
& Perplexity            & $28.67{\scriptstyle \pm 9.34}$ & $9.38{\scriptstyle \pm 8.95}$ & $24.16{\scriptstyle \pm 2.45}$ & $35.19{\scriptstyle \pm 10.99}$ & $14.5{\scriptstyle \pm 5.98}$ & $5.33{\scriptstyle \pm 6.09}$ \\
& Word-frequency        & \cellcolor{gray!20}$11.43{\scriptstyle \pm 3.0}$ & \cellcolor{gray!20}$7.33{\scriptstyle \pm 6.59}$ & \cellcolor{gray!20}$6.85{\scriptstyle \pm 5.03}$ & $3.44{\scriptstyle \pm 4.61}$ & $0{\scriptstyle \pm 0}$ & $6.6{\scriptstyle \pm 9.35}$ \\
\midrule
\multirow{4}{*}{Pythia-v0}
& Direct asking         & -- & -- & -- & -- & -- & -- \\
& BB generation         & $46.75{\scriptstyle \pm 3.64}$ & $23.45{\scriptstyle \pm 5.89}$ & $10.31{\scriptstyle \pm 4.85}$ &\cellcolor{gray!20} $3.56{\scriptstyle \pm 2.03}$ & \cellcolor{gray!20} $ 5.61{\scriptstyle \pm 0.78}$ & \cellcolor{gray!20} $2.15{\scriptstyle \pm 2.45}$ \\
& Perplexity            & $22.33{\scriptstyle \pm 15.8}$ & $11.25{\scriptstyle \pm 13.68}$ & $25.79{\scriptstyle \pm 15.59}$ & $4.32 {\scriptstyle \pm 3.25}$ & $9.94 {\scriptstyle \pm 0.59}$ & $9.39 {\scriptstyle \pm 0}$ \\
& Word-frequency        & \cellcolor{gray!20}$22{\scriptstyle \pm 10.4}$ & \cellcolor{gray!20}$7.95{\scriptstyle \pm 9.44}$ & \cellcolor{gray!20}$9.25{\scriptstyle \pm 11.9}$ & $3.31{\scriptstyle \pm 4.68}$ & $3.27{\scriptstyle \pm 4.62}$ & $6.73{\scriptstyle \pm 8.22}$ \\
\midrule
\multirow{4}{*}{Llama-3}
& Direct asking         & $14.27{\scriptstyle \pm 5.32}$ & $4.86{\scriptstyle \pm 1.33}$ & $19.9{\scriptstyle \pm 4.24}$ & $17.97{\scriptstyle \pm 5.33}$ & $4.0{\scriptstyle \pm 2.12}$ & $16.17{\scriptstyle \pm 1.18}$ \\
& BB generation         & $23.64{\scriptstyle \pm 5.82}$ & $5.79{\scriptstyle \pm 6.46}$ & $14.01{\scriptstyle \pm 1.68}$ & \cellcolor{gray!20}$0.61{\scriptstyle \pm 0.77}$ & \cellcolor{gray!20}$1.33{\scriptstyle \pm 1.31}$ & \cellcolor{gray!20}$1.25{\scriptstyle \pm 1.52}$ \\
& Perplexity            & $13.28{\scriptstyle \pm 4.77}$ & $25.0{\scriptstyle \pm 25.4}$ & $19.01{\scriptstyle \pm 20.52}$ & $17.80{\scriptstyle \pm 9.06}$ & $19.85{\scriptstyle \pm 7.6}$ & $6.24{\scriptstyle \pm 7.57}$ \\
& Word-frequency        & \cellcolor{gray!20}$8.29{\scriptstyle \pm 2.13}$ & \cellcolor{gray!20}$7.33{\scriptstyle \pm 6.59}$ & \cellcolor{gray!20}$10.66{\scriptstyle \pm 7.12}$ & $2.45{\scriptstyle \pm 2.3}$ & $3.33{\scriptstyle \pm 4.7}$ & $5.83{\scriptstyle \pm 1.73}$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Attack Performance for gender property in the QA mode (left) and Chat-Completion mode (right).} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio.}
\label{tab:gender}
\end{table}


\begin{table}[ht]
\centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc}
\toprule
\textbf{Model} & \textbf{Attacks} & \multicolumn{3}{c|}{\textbf{QA Mode}} & \multicolumn{3}{c}{\textbf{Chat-Completion Mode}} \\
              &                   & Mental & Digestive & Childbirth & Mental & Digestive & Childbirth \\
\midrule
\multirow{3}{*}{Llama-1}
& Generation w/o FT     & 3.45 & 4.19 & 9.88 & 3.45 & 4.19 & 9.88 \\
& Direct asking         & $7.66{\scriptstyle \pm 2.05}$ & $0.18{\scriptstyle \pm 0}$ & $9.2{\scriptstyle \pm 0}$ & $8.62{\scriptstyle \pm 2.36}$ & $0.17{\scriptstyle \pm 0}$ & $9.2{\scriptstyle \pm 0}$ \\
& BB generation         & \cellcolor{gray!20}$2.55{\scriptstyle \pm 0.25}$ & \cellcolor{gray!20}$3.94{\scriptstyle \pm 0.37}$ & \cellcolor{gray!20}$7.95{\scriptstyle \pm 0.36}$ & \cellcolor{gray!20}$1.76{\scriptstyle \pm 0.23}$ & \cellcolor{gray!20}$1.44{\scriptstyle \pm 0.24}$ & \cellcolor{gray!20}$6.99{\scriptstyle \pm 0.18}$ \\
\midrule
\multirow{3}{*}{Pythia-v0}
& Generation w/o FT     & 1.84 & 9.57 & 9.85 & 1.84 & 9.57 & 9.85 \\
& Direct asking         & -- & -- & -- & -- & -- & -- \\
& BB generation         & \cellcolor{gray!20}$1.82{\scriptstyle \pm 0.56}$ & \cellcolor{gray!20}$3.71{\scriptstyle \pm 0.82}$ & \cellcolor{gray!20}$7.63{\scriptstyle \pm 0.31}$ & \cellcolor{gray!20}$1.88{\scriptstyle \pm 0.36}$ & \cellcolor{gray!20}$1.84{\scriptstyle \pm 0.16}$ & \cellcolor{gray!20}$6.23{\scriptstyle \pm 0.52}$ \\
\midrule
\multirow{3}{*}{Llama-3}
& Generation w/o FT     & 3.45 & 4.64 & 10.32 & 3.45 & 4.64 & 10.32 \\
& Direct asking         & $19.96{\scriptstyle \pm 17.74}$ & $14.22{\scriptstyle \pm 0}$ & $10.26{\scriptstyle \pm 0.47}$ & $5.03{\scriptstyle \pm 0}$ & $12.64{\scriptstyle \pm 0}$ & $10.27{\scriptstyle \pm 0.5}$ \\
& BB generation         & \cellcolor{gray!20}$1.43{\scriptstyle \pm 0.7}$ & \cellcolor{gray!20}$1.80{\scriptstyle \pm 1.18}$ & \cellcolor{gray!20}$7.73{\scriptstyle \pm 0.38}$ & \cellcolor{gray!20}$0.63{\scriptstyle \pm 0.23}$ & \cellcolor{gray!20}$1.82{\scriptstyle \pm 0.45}$ & \cellcolor{gray!20}$4.59{\scriptstyle \pm 0.35}$ \\
\bottomrule
\end{tabular}}
\caption{\textbf{Attack Performance for medical diagnosis in the QA mode (left) and Chat-Completion mode (right).} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio.}
\label{tab:medical}
\end{table}


% Previous tables
% \begin{table}[htbp]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{3}{c}{\textbf{Target gender ratios}} \\
% \cmidrule(lr){3-5}
%  &  & \textbf{30} & \textbf{50} & \textbf{70} \\
% \midrule
% \multirow{4}{*}{Llama-1} & Direct asking & $\underline{23.17 {\scriptstyle \pm 1.78}}$ & $\textbf{3.98} {\scriptstyle \pm 1.88}$ & $18.6{\scriptstyle \pm 0}$ \\
%  & Black-box generation & $36.52 {\scriptstyle \pm 0.11}$ & $15.45 {\scriptstyle \pm 3.09}$ & $\textbf{1.45} {\scriptstyle \pm 0.64}$ \\
%  & Perplexity-attack & $28.67 {\scriptstyle \pm 9.34}$ & $9.38 \pm 8.95$ & $24.16 {\scriptstyle \pm 2.45}$\\
%  & Word-frequency attack & $\textbf{11.43} {\scriptstyle \pm 3.0}$ & $\underline{7.33 {\scriptstyle \pm 6.59}} $ & $\underline{6.85 {\scriptstyle \pm 5.03}}$ \\
% \midrule
% \multirow{4}{*}{Pythia-v0} & Direct asking & -- & -- & -- \\
%  & Black-box generation & $46.75 {\scriptstyle \pm 3.64}$ & $23.45 {\scriptstyle \pm 5.89}$ & $\underline{10.31 {\scriptstyle \pm 4.85}}$ \\
%  & Perplexity-attack & $\underline{22.33 {\scriptstyle \pm 15.8}}$ & $\underline{11.25 {\scriptstyle \pm 13.68}}$ & $25.79 {\scriptstyle \pm 15.59}$ \\
%  & Word-frequency attack & $\textbf{22} {\scriptstyle \pm 10.4}$ & $\textbf{7.95} {\scriptstyle \pm 9.44}$ & $\textbf{9.25} {\scriptstyle \pm 11.9}$ \\
% \midrule
% \multirow{4}{*}{Llama-3} & Direct asking & $14.27 {\scriptstyle \pm 5.32}$ & $\textbf{4.86} {\scriptstyle \pm 1.33}$ & $19.9 {\scriptstyle \pm 4.24}$ \\
%  & Black-box generation & $23.64 {\scriptstyle \pm 5.82}$ & $\underline{5.79} {\scriptstyle \pm 6.46}$ & $\underline{14.01} {\scriptstyle \pm 1.68}$ \\
%  & Perplexity-attack & $\underline{13.28} {\scriptstyle \pm 4.77}$ & $25.0 {\scriptstyle \pm 25.4}$ & $19.01 {\scriptstyle \pm 20.52}$ \\
%  & Word-frequency attack & $\textbf{8.29} {\scriptstyle \pm 2.13}$ & $7.33 {\scriptstyle \pm 6.59}$ & $\textbf{10.66} {\scriptstyle \pm 7.12}$ \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Attack Performance for gender attribute in the QA mode.} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio. 
% % \cy{changed caption -- use this everywhere; lets call is QA mode rather than QandA everywhere}
% }
% \label{tab: gender; question-answering}
% \end{table}

% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  Target medical ratio &  Mental Disorder  &  Digestive Disorder & Child birth \\
%           % &      &   &    \\
% \hline
% \multicolumn{4}{ |c| }{Llama-1} \\ \hline
% Generation (w/o fine-tuning)  & $3.45$  & $4.19$ & $9.88$\\ \hline
% Baseline 1 (direct asking) &  &  &  \\
% Black-box generation attack  & $2.55 {\scriptstyle\pm 0.25}$   & $3.94 {\scriptstyle\pm 0.37}$  & $7.95 {\scriptstyle\pm 0.36}$ \\  \hline 
% \multicolumn{4}{ |c| }{Pythia} \\
% \hline
% Generation (w/o fine-tuning)  & $1.84$ & $9.57$ & $9.85$\\ \hline
% Baseline 1 (direct asking) & & &  \\
% Black-box generation attack & $1.82 {\scriptstyle \pm 0.56}$  & $3.71 {\scriptstyle \pm 0.82} $ & $7.63 {\scriptstyle \pm 0.31} $ \\  \hline 
% \multicolumn{4}{ |c| }{Llama-3} \\
% \hline
% Generation (w/o fine-tuning)  & $3.45$ & $4.64$ & $10.32$ \\ \hline
% Baseline 1 (direct asking) &  & &  \\
% Black-box generation attack &$1.43 {\scriptstyle \pm 0.7}$  & $1.80 {\scriptstyle\pm 1.18}$ & $7.73{\scriptstyle\pm 0.38}$ \\  \hline 
% \end{tabular}
% \end{center}
% \caption{Attack performance for medical diagnosis in the QA mode. 
% We report the mean and standard deviation of the absolute average difference between the predicted attribute and the target attribute. Note that the reported number is close to 0 indicates that the adversary can accurately infer this target attribute.}
% \label{tab: medical;quesiton-answering}
% \end{table}



% \begin{table}[htbp]
% \centering
% \label{tab:attack-results}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{3}{c}{\textbf{Attributes}} \\
% \cmidrule(lr){3-5}
%  &  & \textbf{Mental Disorder} & \textbf{Digestive Disorder} & \textbf{Childbirth} \\
% \midrule
% \multirow{4}{*}{Llama-1} 
% & Generation w/o FT & $3.45$  & $4.19$ & $9.88$\\
% % & Direct asking & $8.63 \pm 2.36$ & $0.18 \pm 0$ & $10.6 \pm 0$ \\
% & Direct asking & $7.66 \pm 2.05$ & $0.18 \pm 0$ & $9.2 \pm 0$ \\
%  & Black-box generation & $2.55 {\scriptstyle\pm 0.25}$   & $3.94 {\scriptstyle\pm 0.37}$  & $7.95 {\scriptstyle \pm 0.36}$ \\
 
% \midrule
% \multirow{4}{*}{Pythia-v0}
% & Generation w/o FT & $1.84$ & $9.57$ & $9.85$ \\
% & Direct asking & -- & -- & -- \\
%  & Black-box generation & $1.82 {\scriptstyle \pm 0.56}$  & $3.71 {\scriptstyle \pm 0.82} $ & $7.63 {\scriptstyle \pm 0.31} $  \\
% \midrule
% \multirow{4}{*}{Llama-3}
% & Generation w/o FT  & $3.45$ & $4.64$ & $10.32$  \\
% & Direct asking & $19.96 {\scriptstyle \pm 17.74}$ & $14.22 {\scriptstyle \pm 0}$ & $10.26 {\scriptstyle \pm 0.47}$ \\
%  & Black-box generation &$1.43 {\scriptstyle \pm 0.7}$  & $1.80 {\scriptstyle\pm 1.18}$ & $7.73{\scriptstyle\pm 0.38}$  \\
% \bottomrule
% \end{tabular}
% \caption{ \textbf{Attack Performance for medical diagnosis in the QA mode.} Reported numbers are the Mean absolute errors between the predicted and target ratios. Lower is better; zero means the predicted ratio exactly matches target ratio.}
% \label{tab: medical;quesiton-answering}
% \end{table}

% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  Target medical ratio &  Mental Disorder  &  Digestive Disorder & Child birth & Abs Diff \\
%           &  5.104\%    & 12.68\%  &  10.6\% & \\
% \hline
% \multicolumn{5}{ |c| }{Llama-1} \\ \hline
% Generation (w/o fine-tuning)  & 1.56   & 7.91 & 0.658 & $6.08 $ \\ \hline
% Baseline 1 (direct asking) & $12.77 \pm 2.05$ & $12.5 \pm 0$ & $1.4 \pm 0$ & $5.68$ \\
% % generated attack (prompt 1) & 6.92  & 9.83  & 2.78 & 4.16 \\
% % generated attack (prompt 2) &  5.60  & 9.63  & 2.02  & \textbf{4.04} \\
% % generated attack (prompt 3) & 9.51  & 7.69 & 2.24 & 5.91\\ 
% Black-box generation attack  & $7.66 \pm 0.25$   & $8.74 \pm 0.37$  & $2.64 \pm 0.36$  & $4.81$ \\  \hline 
% \multicolumn{5}{ |c| }{Pythia} \\
% \hline
% Generation (w/o fine-tuning)  & $3.67$ & $3.10$ & $0.75$  & $6.95$\\ \hline
% Baseline 1 (direct asking) & & & & \\
% % generated attack (prompt 1) &  & &  & \\
% % generated attack (prompt 2) &   &  &  & \\
% % generated attack (prompt 3) &   &  &  & \\ 
% Black-box generation attack & $6.58 \pm 0.97$  & $8.97 \pm 0.82$ & $2.96 \pm 0.31$  & $4.15$ \\  \hline 
% \multicolumn{5}{ |c| }{Llama-3} \\
% \hline
% Generation (w/o fine-tuning)  & $1.65$ & $8.03$ & $0.28$ & $6.14$\\ \hline
% Baseline 1 (direct asking) & $21.67 \pm 20.9$ & $13.34 \pm 15.45$& $0 \pm 0$ & $14.9$ \\
% % generated attack (prompt 1) & 4.81  & 12.09 & 2.29  & 3.03 \\
% % generated attack (prompt 2) & 4.67  & 10.74  & 1.89  & 3.66 \\
% % generated attack (prompt 3) & 5.28  & 13.44 & 3.89  & \textbf{2.57}\\ 
% Black-box generation attack &$5.51 \pm 1.49$  & $11.46 \pm 1.72$ & $2.86 \pm 0.38$ & $3.54$ \\  \hline 
% \end{tabular}
% \end{center}
% \caption{Attack performance for medical diagnosis in the QA mode. The number reported on the second to fourth columns are the average predicted ratio and the standard deviation. The last column is the average absolute different. }
% \label{tab: medical;quesiton-answering}
% \end{table}

% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \multirow{2}{*}{5}  target medical ratio &  Mental Disorder  &  Digestive Disorder & Child birth & Absolute Diff \\
%          &  5.104\%    & 12.68\%  &  10.6\% &  \\
% \hline
% \multicolumn{5}{ |c| }{Llama-1} \\
% \hline

% generated attack (prompt 1) & 0.7  & 6.69 & 0.704 & 6.75  \\
% generated attack (prompt 2) & 1.18  & 7.41 & 0.69  & 6.36\\
% generated attack (prompt 3) & 2.8  & 9.63 & 0.58  &  5.12\\ 
% generated attack (average) & 1.56   & 7.91 & 0.658 & \\  \hline 
% \multicolumn{5}{ |c| }{Pythia} \\
% \hline
% generated attack (prompt 1) &   &  &  & \\
% generated attack (prompt 2) &   &  &  & \\
% generated attack (prompt 3) &   &  &  & \\ 
% generated attack (average) &   &  &  & \\  \hline 
% \multicolumn{5}{ |c| }{Llama-3} \\
% \hline
% generated attack (prompt 1) & 0.74  & 6.22  & 0.06 & 7.2 \\
% generated attack (prompt 2) &   &  &  & \\
% generated attack (prompt 3) &   &  &  & \\ 
% generated attack (average) &   &  &  & \\  \hline 
% \end{tabular}
% \end{center}
% \caption{Attack performance for medical diagnosis with model without fine-tuning. The number reported on the second to fourth columns are the average predicted ratio and the standard deviation. The last column is the average absolute different. }
% \label{tab: before-fine tuning}
% \end{table}


\subsection{Observations from Chat-Completion mode}
%\textbf{In the chat-completion mode, both our word-frequency-based shadow attack and the black-box generation attack achieve effective performance in inferring gender property.} As demonstrated in Table \ref{tab:Gender;chat-completion}, the average absolute difference is $2 \% - 4\%$.  We think the reason is that the model learns the joint probability distribution of both the inputs and the outputs, as described in Equation \ref{Training objective 2}, hence the generated texts mirrors the fine-tuning dataset's word distribution. 

\textbf{For the gender property, both our word-frequency-based shadow attack and the black-box generation attack achieve effective performance.} As demonstrated in Table \ref{tab:Gender;chat-completion}, both the black-box generation attack and the word-frequency shadow attack achieve very low error across different targets; for instance the smallest error achieved by the black-box generation attack is $0.61\%$ while the word-frequency attack predicts some target ratios perfectly with zero error \cy{is this correct?}.  The reason for this success is likely that the model learns the \textit{joint} probability distribution of both the inputs and the outputs (as opposed to the conditional distribution in the QA mode), as described in Equation \ref{Training objective 2}, which allows the generated texts to mirror the word distribution of the fine-tuning dataset. These attacks also perform better than the baselines, for similar reasons as mentioned in the QA mode.

\textbf{The fine-tuning methodology has an impact on the performance of the attacks.} While the black-box generation attack did not have discriminative power between different target ratios in the QA mode (Table \ref{tab: gender; question-answering}), it does have it in the chat-completion mode as is evident from small errors across different target ratios. Additionally, the word-frequency shadow attack also has more successful attack performance in the chat-completion mode as compared to QA mode, as is evident by smaller errors in the chat-completion mode. We believe the reason for this gain is that different fine-tuning methods correspond to different memorization patterns, some of which can be more amenable for property inference.

\textbf{For medical diagnosis properties, the black-box generation attack achieves effective performance.} Similar to QA mode, the black-box generation attack achieves the best performance in inferring medical diagnosis property ratios, as it evident by the lowest errors achieved by this attack across the board \ref{tab:medical;chat-completion}. The error for childbirth is again much higher than the other two properties for similar reasons as the QA mode.


%\textbf{Fine-tuning method have an impact on the performance of the attacks.} Compared to the attack results in Q\&A mode (Table \ref{tab:Gender;chat-completion}), where the black-box generation attack does not have discriminative power between different target ratios, the black-box generation attack has effective performance in the chat-completion mode -- as we can see the absolute average difference in the Q\&A mode is above $14\%$, whereas the absolute average difference in the chat-completion mode is less than $3\%$. In addition, the word-frequency-based shadow model attack also has more successful attack performance in the chat-completion mode -- the absolute average difference in the Q\&A mode is $7-11\%$ and the absolute average difference in the chat-completion mode is between $2-5\%$.  We think the reason is that different fine-tuning methods correspond to different memorization patterns. 


% Table \ref{tab:Gender;chat-completion} shows the attack results for the patient's gender property: for each target ratio $\{0.3, 0.5, 0.7 \}$, we report the mean and standard deviation of the predicted ratio between different random seed; for each attack, we also report the absolute average different between the target ratio and the predicted ratio. In general, the black-box generation attack and the shadow model attack based on word frequency have good attack performance; the average absolute difference for these two attacks is less than $5\%$. For black-box generation attack, we observe that there is not a single input text that achieves the best performance among all models, instead averaging different input-texts has the overall best performance.
% On the other hand, the baseline attacks and the shadow model attack based on perplexity .... \ph{Todo: add baseline attack results.}.

% To consider the effect of pre-training, table \ref{tab: before-fine tuning} shows the predicted ratio of the medical diagnosis without fine-tuning; table \ref{tab:Med:chat-completion} shows the attack results for the properties of the medical diagnosis after fine-tuning, we report the mean and standard deviation of the predicted ratio; for each attack, we also report the average absolute difference between the target ratio and the predicted ratio. We only test the black-box access attacks for this property -- since we do not subsample the fine-tuning due to data limitation, and if the adversary has access to auxiliary data, the adversary is able to directly estimate the target ratio using the auxiliary data, which makes this problem trivial.
%\textbf{In the chat-completion mode, the black-box generation attack achieves effective performance in inferring medical diagnosis property.}
%The result shows that the black-box generation attack has high accuracy in mental disorder and digestive disorder, for example, the target ratio of mental disorder and digestive disorder is $5.104\% $ and $12.68\% $, respectively, and the predicted ratio of Llama-1 is $5.53\% $ and $12.05\% $, respectively, where the difference is less than $1 \%$. The predicted ratio for childbirth is quite far away from the target ratio; we suspect this is because childbirth, such as birth-control, is a culturally sensitive topic, and the models may have done some pre-training or alignment training that reduce the likelihood of outputting childbirth-related content. 

% Previous tables
% \begin{table}[htbp]
% \centering
% \label{tab:attack-results}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccc}
% \toprule
% \multirow{2}{*}{\textbf{Target model}} & \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{3}{c}{\textbf{Target gender ratios}} \\
% \cmidrule(lr){3-5}
%  &  & \textbf{30} & \textbf{50} & \textbf{70} \\
% \midrule
% \multirow{4}{*}{Llama-1} & Direct asking & $22.8 {\scriptstyle \pm 1.98}$ & $7.7 {\scriptstyle \pm 1.8}$ & $18.57 {\scriptstyle \pm 4.71}$ \\
%  & Black-box generation & $1.73 {\scriptstyle \pm 0.76}$ & $2.64 {\scriptstyle \pm 3.33}$ & $3.28 {\scriptstyle \pm 3.64}$  \\
%  & Perplexity-attack & $35.19 {\scriptstyle \pm 10.99}$ & $14.5 {\scriptstyle \pm 5.98}$ & $5.33 {\scriptstyle \pm 6.09}$ \\
%  & Word-frequency attack & $10 {\scriptstyle \pm 0}$ & $0 {\scriptstyle \pm 0}$ & $0 {\scriptstyle \pm 0}$ \\
% \midrule
% \multirow{4}{*}{Pythia-v0} & Direct asking & -- & -- & -- \\
%  & Black-box generation & $3.56 {\scriptstyle \pm 2.03}$ & $5.61 {\scriptstyle \pm 0.78}$ & $2.15 {\scriptstyle \pm 2.45}$\\
%  & Perplexity-attack &  & &  \\
%  & Word-frequency attack & $3.31 {\scriptstyle \pm 4.68}$ & $3.27 {\scriptstyle \pm 4.62}$ & $6.73 {\scriptstyle \pm 8.22}$ \\
% \midrule
% \multirow{4}{*}{Llama-3} & Direct asking & $17.97 {\scriptstyle \pm 5.33}$ & $4.0 {\scriptstyle \pm 2.12}$ & $16.17 {\scriptstyle \pm 1.18}$\\
%  & Black-box generation & $0.61 {\scriptstyle \pm 0.77}$ & $1.33 {\scriptstyle \pm 1.31}$ & $1.25 {\scriptstyle \pm 1.52}$ \\
%  & Perplexity-attack & $17.80 {\scriptstyle \pm 9.06}$ & $19.85 {\scriptstyle \pm 7.6}$ & $6.24 {\scriptstyle \pm 7.57}$\\
%  & Word-frequency attack & $3.31 {\scriptstyle \pm 4.68}$ & $8.05 {\scriptstyle \pm 8.11}$ & $6.78 {\scriptstyle \pm 5.23}$\\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Attack Performance for gender attribute in the Chat-Completion mode.} We report the MAE (mean absolute error) between the predicted ratio and the target ratio. The reported number is close to 0 indicates that the adversary can accurately infer this target attribute.}
% \label{tab:Gender;chat-completion}
% \end{table}


% \begin{table}[htbp]
% \centering
% \label{tab:attack-results}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccc}
% \toprule
% \multirow{2}{*}{\textbf{Target model}} & \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{3}{c}{\textbf{Attributes}} \\
% \cmidrule(lr){3-5}
%  &  & \textbf{Mental Disorder} & \textbf{Digestive Disorder} & \textbf{Childbirth} \\
% \midrule
% \multirow{4}{*}{Llama-1} 
% & Generation w/o FT & $3.45$  & $4.19$ & $9.88$\\
% % & Direct asking & $8.63 \pm 2.36$ & $0.18 \pm 0$ & $10.6 \pm 0$ \\
% & Direct asking  & $8.62 {\scriptstyle \pm 2.36}$  & $0.17 {\scriptstyle \pm 0}$ & $9.2 {\scriptstyle \pm 0}$\\
%  & Black-box generation   &  $1.76 {\scriptstyle \pm 0.23}$ & $1.44 {\scriptstyle \pm 0.24}$ & $6.99 {\scriptstyle \pm 0.18}$ \\
 
% \midrule
% \multirow{4}{*}{Pythia-v0}
% & Generation w/o FT & $1.84$ & $9.57$ & $9.85$ \\
% & Direct asking & -- & -- & -- \\
%  & Black-box generation  & $1.82 {\scriptstyle \pm 0.56}$ & $3.71 {\scriptstyle \pm 0.82}$ & $7.64 {\scriptstyle \pm 0.31}$ \\
% \midrule
% \multirow{4}{*}{Llama-3}
% & Generation w/o FT  & $3.45$ & $4.64$ & $10.32$  \\
% & Direct asking & $5.03 \pm 0$ & $12.64 \pm 0$ & $10.27 \pm 0.5$ \\
%  & Black-box generation  & $0.63 {\scriptstyle \pm 0.23}$  & $1.80 {\scriptstyle \pm 1.18}$ & $7.73 {\scriptstyle \pm 0.38}$\\
% \bottomrule
% \end{tabular}
% \caption{ \textbf{Attack Performance for medical diagnosis in the Chat-Completion mode.} We report the MAE (mean absolute error) between the predicted attribute and the target attribute. Note that the reported number is close to 0 indicates that the adversary can accurately infer this target attribute.}
% \label{tab:medical;chat-completion}
% \end{table}

% \begin{table}[h!] 
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
% Target female ratio  ( \%) = &  30 &  50 & 70 & Abs diff \\ 
% \hline
% \multicolumn{5}{ |c| }{Llama-1} \\
% \hline
% Baseline 1 (direct asking) & $52.8 \pm 1.97$  & $57.70 \pm 1.80$  & $51.43 \pm 0.05$  & $16.36$ \\  
% % generated attack (prompt 1) &  $33.7 \pm 1.8$ & $55 \pm 2.6$ & $71.8 \pm 3.6$ & $4.1$  \\
% % generated attack (prompt 2) & $30 \pm 4$  & $50 \pm 5$ & $68 \pm 5$ & $4.4$ \\
% % generated attack (prompt 3) & $29.6 \pm 1.3$ & $48.3 \pm 2.6$ & $69.6 \pm 2.4$ & $\textbf{2.1}$ \\ 
% Black-box generation attack & $31.20 \pm 1.47$ & $51.35 \pm 3.33$ & $69.91 \pm 3.64$ & $2.55$ \\ 
% % shadow model attack (prompt 1) & $0.469 \pm 0.084 $ & $0.515 \pm 0.019$ & $0.612 \pm 0.075$ & 0.091 \\
% % shadow model attack (prompt 2) & $0.472 \pm 0.038$ & $0.533 \pm 0.047$ & $0.618 \pm 0.024$ & 0.095  \\
% % shadow model attack (prompt 3) &  $0.442 \pm 0.043$ & $0.584 \pm 0.038$ & $0.559 \pm 0.14$ & 0.122  \\
% Shadow model attack (loss)  &  &  &  & \\ 
% Shadow model attack (word frequency) & $33 \pm 4$  & $43 \pm 4.7$  & $70 \pm 0$ & $3.4$  \\ \hline

% \multicolumn{5}{ |c| }{Pythia-v0-6.9b} \\
% \hline  
% Baseline 1 (direct asking) &  &  &  & \\  
% % generated attack (prompt 1) &  $26.8 \pm 5$ & $56.6 \pm 2$ & $71.6 \pm 2$ & $4.7$  \\
% % generated attack (prompt 2) & $27.6 \pm 3$  & $53.9 \pm 2$ & $69.8 \pm 3$ & $3.3$ \\
% % generated attack (prompt 3) & $34 \pm 4$ & $56 \pm 0.3$ & $74.9 \pm 2.7$ & $ 5$ \\ 
% Black-box generation attack & $29.62 \pm 4.08$ & $55.61 \pm 0.77$ & $72.15 \pm 2.45$ & $3.77$ \\   
% % shadow model attack (prompt 1) & $0.469 \pm 0.084 $ & $0.515 \pm 0.019$ & $0.612 \pm 0.075$ & 0.091 \\
% % shadow model attack (prompt 2) & $0.472 \pm 0.038$ & $0.533 \pm 0.047$ & $0.618 \pm 0.024$ & 0.095  \\
% % shadow model attack (prompt 3) &  $0.442 \pm 0.043$ & $0.584 \pm 0.038$ & $0.559 \pm 0.14$ & 0.122  \\
% Shadow model attack (loss)  &  &  &  & \\
% Shadow model attack (word frequency) & $26 \pm 4.6$  & $50 \pm 0$ & $66.6 \pm 4.7$  & $\textbf{2.2}$  \\ \hline

% \multicolumn{5}{ |c| }{Llama-3-8b-instruct} \\
% \hline
% Baseline 1 (direct asking) & $47.97 \pm 5.33$  & $54 \pm 2.12$  & $53.83 \pm 1.18$  & $12.71$ \\ 
% % generated attack (prompt 1) &  $31.9 \pm 1.1$ & $50.8 \pm 1.4$ & $71.7 \pm 1.6$ & 1.8  \\
% % generated attack (prompt 2) & $29.4 \pm 1.1$  & $50.4 \pm 2.2$ & $70.2 \pm 2.4$ & 1.8 \\
% % generated attack (prompt 3) & $26.8 \pm 0.4$ & $44.8 \pm 2.4$ & $67.2\pm 1.4$ & 3.7 \\ 
% Black-box generation attack & $29.41 \pm 0.78$ & $48.67 \pm 1.31$ & $69.73 \pm 1.52$ & \textbf{1.06} \\
% % shadow model attack (prompt 1) & $0.469 \pm 0.084 $ & $0.515 \pm 0.019$ & $0.612 \pm 0.075$ & 0.091 \\
% % shadow model attack (prompt 2) & $0.472 \pm 0.038$ & $0.533 \pm 0.047$ & $0.618 \pm 0.024$ & 0.095  \\
% % shadow model attack (prompt 3) &  $0.442 \pm 0.043$ & $0.584 \pm 0.038$ & $0.559 \pm 0.14$ & 0.122  \\
% Shadow model attack (loss) &  &  &  & \\  
% Shadow model attack (word frequency) &  &  & &  \\ \hline
% \end{tabular}
% \end{center}
% \caption{Attack performance for gender with model fine-tuned with Chat-Completion mode. The number reported on the second to fourth columns are the mean and standard deviation of the predicted ratio. The last column is the average absolute difference of each attack. }
% \label{tab:Gender;chat-completion}
% \end{table}


% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  \multirow{2}{*}{5}  target medical ratio &  Mental Disorder  &  Digestive Disorder & Child birth \\
% \hline
% \multicolumn{4}{ |c| }{Llama-1} \\
% \hline
% Generation (w/o fine-tuning)  & $3.45$  & $4.19$ & $9.88$\\ \hline
% Baseline (direct asking) &   &  &  \\ 
% Black-box generated attack & $1.76 {\scriptstyle \pm 0.23}$  & $1.14 {\scriptstyle \pm 0.24}$  & $6.99 {\scriptstyle \pm 0.18}$  \\  \hline 
% \multicolumn{4}{ |c| }{Pythia-v0-6.9b} \\
% \hline
% Generation (w/o fine-tuning)  & $1.84$ & $9.57$ & $9.85$\\ \hline
% baseline (direct asking) & & & \\  
% generated attack (average) & $1.88 {\scriptstyle \pm 0.36}$  & $1.83 {\scriptstyle \pm 0.16}$  & $6.23 {\scriptstyle \pm 0.53}$  \\  \hline 
% \multicolumn{4}{ |c| }{Llama-3-8b-instruct} \\
% \hline
% Generation (w/o fine-tuning)  & $3.45$ & $4.64$ & $10.32$ \\ \hline
% baseline (direct asking) &  &  & \\
% generated attack (average) & $0.64 {\scriptstyle \pm 0.7}$ & $1.44 {\scriptstyle \pm 0.24}$ & $6.99 {\scriptstyle \pm 0.18}$ \\  \hline
% \end{tabular}
% \end{center}
% \caption{Attack performance for medical diagnosis with model fine-tuned without input masking (the objective is described in Equation \ref{Training objective 2}) The number reported on the second to fourth columns are the average predicted ratio and the standard deviation. The last column is the average absolute different. }
%  \label{tab:Med:chat-completion}
% \end{table}


% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \multirow{2}{*}{5}  target medical ratio &  Mental Disorder  &  Digestive Disorder & Child birth & Abs Diff \\
%          &  5.104 (\%)    & 12.68 (\%)  &  10.6 (\%) &  \\
% \hline
% \multicolumn{5}{ |c| }{Llama-1} \\
% \hline
% Baseline (direct asking) & $13.73 \pm 2.35$ & $12.5 \pm 0$ & $0 \pm 0$ & $6.47$ \\ 
% % generated attack (prompt 1) & 4.70  & 12.81 & 2.63 & 2.83 \\
% % generated attack (prompt 2) & 3.07  & 14.03 & 4.75 & 3.076 \\
% % generated attack (prompt 3) &  8.86 & 9.32  & 3.84 & 4.63 \\ 
% Black-box generated attack & $5.27 \pm 0.30$  & $12.35 \pm 0.26$  & $3.61 \pm 0.19$  & $2.51$ \\  \hline 
% \multicolumn{5}{ |c| }{Pythia-v0-6.9b} \\
% \hline
% baseline (direct asking) & & & & \\ 
% % generated attack (prompt 1) &   &  &  & \\
% % generated attack (prompt 2) &   &  &  & \\
% % generated attack (prompt 3) &   &  &  & \\ 
% generated attack (average) &  $4.64 \pm 0.41$ & $14.5 \pm 0.16$ & $4.36 \pm 0.52$  & $2.87$ \\  \hline 
% \multicolumn{5}{ |c| }{Llama-3-8b-instruct} \\
% \hline
% baseline (direct asking) & $3.33 \pm 4.71$ & $0 \pm 0$ & $0.33 \pm 0.47$& $9.31$\\
% % generated attack (prompt 1) & 5.2  & 13.6 & 3.90 & 2.57 \\
% % generated attack (prompt 2) & 5.22  & 13.22 & 8.17 & \textbf{1.03}\\
% % generated attack (prompt 3) & 6.17  & 14.06 & 6.61 & 2.14 \\ 
% generated attack (average) & $5.29 \pm 0.35$ & $14.5 \pm 0.45$ & $6.0 \pm 0.35$& $2.23$\\  \hline
% \end{tabular}
% \end{center}
% \caption{Attack performance for medical diagnosis with model fine-tuned without input masking (the objective is described in Equation \ref{Training objective 2}) The number reported on the second to fourth columns are the average predicted ratio and the standard deviation. The last column is the average absolute different. }
%  \label{tab:Med:chat-completion}
% \end{table}




% Separate subsections for Generation and Question-Answering

% - Setup: fine-tuning parameters
% - Attacks: .....
% - Results: Tables/figures
% - Observations:

% Discussion:



==> sections/genattack_chhavi.tex <==
\subsection{Generation-based Attack under Black-Box Access}\label{subsec:genattack}
% \subsection{Generation based attack}
Prior work \cite{zhou2021propertyinferenceattacksgans} has proposed an output generation-based attack for property inference under black-box access. However, this attack was proposed for unconditional GAN models and takes latent codes as input to generate outputs. For LLMs which are conditional generation models, we adapt the attack to generate outputs based on input prompts.


Our attack, following \cite{zhou2021propertyinferenceattacksgans}, relies on the distribution of the generated output samples from the target model based on the intuition that the distribution of generated samples from a model can reflect the distribution of the fine-tuning data (in the absence of measures such as constrained decoding that change the output distribution).



%In the black-box setting where the adversary only has API access to the target model, we propose a generation-based attack following \cite{zhou2021propertyinferenceattacksgans}. This attack relies on the distribution of the generated output samples from the target model based on the intuition that the distribution of generated samples from a model can reflect the distribution of the fine-tuning data (in the absence of measures such as constrained decoding that change the output distribution).

%The attack by \cite{zhou2021propertyinferenceattacksgans} is meant for unconditional GAN models and takes latent codes as input to generate outputs. For LLMs which are conditional generation models, we adapt the attack to generate outputs based on input prompts.


%This attack relies on the distribution of the generated output samples from the target model for property inference, based on the intuition that the distribution of generated samples from a model can reflect the distribution of the fine-tuning data (in the absence of measures such as constrained decoding that change the output distribution) \cite{}. \cy{zhou unconditional models, adapt to llms, to adapt which is what you do.. prompt based, how you choossee the prompt, prompt should be well-selected based on the dataset.}

The attack works as follows : adversary queries the target model  with its designed prompt multiple times, collecting a set of generated outputs, $\mathcal{G}_{prompt} = \{\mathcal{G}_i\}_{i=1}^g$ where $g$ denotes the total number of generations. Then it labels each generated output based on whether the generated output satisfies the property to be inferred or not, leading to the set of labels $\{\hat{P}_i \}_{i=1}^g$ where $\hat{P}_i \in \{ 0, 1, N/A \}$ indicates whether the generated sample $\mathcal{G}_i$ satisfies the property $(\{ 0, 1\})$ or the property does not apply (N/A). For example, if the target property is the gender ratio, $\hat{P}_i = 1$ means that the generated sample $\mathcal{G}_i$ describes a female patient; $\hat{P}_i = 0$ means that $\mathcal{G}_i$ describes a male patient, and $\hat{P}_i = N/A$ means that $\mathcal{G}_i$ is not patient descriptions or does not indicate gender.

The average of these labels is the estimated value of the property \textit{with respect to the input prompt} and is given as,
$$\hat{P}_{\mathcal{G}_{prompt}} = \frac{1}{|\{i: \hat{P}_i \in \{0,1 \} \}|} \sum_{i:\hat{P}_i \in \{0,1 \} }\hat{P}_i$$

The adversary can either consider this average to be its final estimate $\hat{P}$ or average over multiple input prompts leading to the final estimate of the property, given by $\hat{P} = \frac{1}{p} \sum_{j=1}^{p}\hat{P}_{\mathcal{G}_{prompt_j}}$.


The input prompt plays an important role in determining success of the attack and should be selected carefully. We explore different variants of the input prompt, such as those which include the finetuning dataset name `ChatDoctor' and others which just say `doctor', as mentioned in Sec.\ref{subsec:expattacksetup}. For a detailed ablation study on prompts, please see Sec.\ref{subsec:ablation}.

==> sections/intro.tex <==
\section{Introduction}

Current large language models (LLMs) are widely used in various real-world applications, including healthcare \cite{he2025surveylargelanguagemodels}, finance \cite{li2024largelanguagemodelsfinance} and law \cite{lai2023largelanguagemodelslaw}. These models are usually pre-trained or fine-tuned on confidential datasets and made public to assist with some domain-specific task, such as customer-related services, or document summarizations. The privacy issue of the confidential dataset raises an important concern. 
Many studies have shown that LLMs can leak unintended information about the training data. For example, \cite{carlini2019secretsharerevaluatingtesting, carlini2021extractingtrainingdatalarge} shows that one can extract individual's sensitive information, such as email, phone number or social security number, from the training samples.
% Hence, it is important to investigate to what degree the confidential information about the training data is leaked by the LLM models. 
% For example, data extraction attack \cite{carlini2021extractingtrainingdatalarge} and membership inference attack evaluate whether LLMs may leak information about individual training examples.
% Dataset inference evaluate whether a dataset is included in the training samples.\cite{maini2024llmdatasetinferencedid}
% shows that one can recover individual training examples by querying the language model. 
% [talks about general privacy issue here to bridge this]

Property inference \cite{ateniese2013hackingsmartmachinessmarter}, or distribution inference, refers to learning statistical properties (rather than individual training data) of the training data given access to the model trained on it and some auxiliary data. 
Property inference focuses on more macro-level properties of the training data. 
For example, the proportion of patients with mental disorders, political preference of articles are considered sensitive information of the data owner, and leaking these confidential information is a privacy violation.

% Property inference attack is first introduced by \cite{ateniese2013hackingsmartmachinessmarter}. 

Literature has majorly focused on traditional machine learning models, such as the regression model \cite{ateniese2013hackingsmartmachinessmarter}, image classification models \cite{ suri2022formalizingestimatingdistributioninference, suri2024dissectingdistributioninference}, and GANs on images \cite{zhou2021propertyinferenceattacksgans}, however, it remains unclear if property inference continues to be a problem for current LLMs.


% First paragraph: LLM and many privacy threats (e.g. MIA, attribute, data ext);
% Second paragraph: property inference is an important threat (cite all these papers) and has been studied for image and tabular data. In this paper, We study property inference attack for LLM -- exact threat scenarios from property inference in LLMs.


% \item However, previous work in property inference looks at simpler models, such as classification, regression models (and GANs), and simple single properties. It is unclear how to extend these attacks to the larger models of today, such as large language models. (...reasons..) Consequently, it is unclear if property inference continues to be a problem for LLMs, which are frequently trained or fine-tuned on confidential and sensitive data. 

% Previous works have shown that property inference attacks success on traditional machine learning architecture, including support vector machines and hidden Markov models \cite{ateniese2013hackingsmartmachinessmarter}, fully connected neural networks \cite{ganju2018property} convolutional neural networks \cite{ suri2022formalizingestimatingdistributioninference, suri2024dissectingdistributioninference} and generative adversarial model (GANs) \cite{zhou2021propertyinferenceattacksgans}. Its success has proven that there is a privacy leakage for these traditional models. However, it remains unclear if property inference continues to be a problem for current LLMs.

In this work, we propose a benchmark task for measuring property inference in LLMs. Specifically, we design a scenario where the LLM's original task is question answering for healthcare, and the adversary's task is to infer patient's distribution, such as the ratio of female, and some sensitive disease's distribution, such as the ratio of patients with mental disorder. 
Here, the threat is realistic since the adversary can act as a customer to steal the distribution of patients' symptoms, which is a clear privacy leakage for the hospitals.
We emphasize that the original task of the LLM is independent of the sensitive information that the adversary is trying to infer. 
We use the ChatDoctor dataset \cite{li2023chatdoctormedicalchatmodel} as the task dataset, which consists of 100k patient-doctor conversation. We augment the dataset by labeling the data with gender and specific diseases, including mental disorder, childbirth, allergy or digestion issue. 
% we propose a medical dataset (...) ... sensitive properties [Goal: Make it sound like this is a problem.] We augment the dataset with labels ...

We evaluate existing attacks on our benchmark. ... We show that auxiliary data based attacks do not work as well. (give one sentence with some numbers)

We propose a simple yet powerful attack as follows: we use some input-text that ask the LLM to generate synthetic patients information and predict the training sample distribution based on the generated-sample distribution. 

Concluding paragraph: (1) Property inference continues to be a problem in LLMs, especially when fine-tuned on confidential data. LLMs are increasingly being fine-tuned on confidential and proprietary information, and people who release LLMs trained on confidential information should be aware that some of the confidential properties may leak out. (2) Prior auxiliary data-based attacks do not work as well on LLMs; instead, simple generation-based attacks work surprisingly well.


==> sections/intro_from_kamalika.tex <==

\section{Introduction}

\begin{itemize}

\item Property inference: convince people that property inference is an important problem. In some cases, this might lead to leakage of confidential information. (Vitaly Shamtikov, Dave Evans).. also mention what it is..[Define property inference: Property inference refers to learning properties of the training data given a model trained on this data and some auxiliary information. Give an example: For example, X shows that the gender ratio can be inferred based on ...]

\item However, previous work in property inference looks at simpler models, such as classification and regression models, and simple single properties. It is unclear how to extend these attacks to the larger models of today, such as large language models. (...reasons..) Consequently, it is unclear if property inference continues to be a problem for LLMs, which are frequently trained or fine-tuned on confidential and sensitive data. 

\item In this work, we propose a benchmark task for measuring property inference in LLMs. Specifically, we propose a medical dataset (...) ... sensitive properties [Goal: Make it sound like this is a problem.] We augment the dataset with labels ...

\item We evaluate existing attacks on our benchmark. ... We show that auxiliary data based attacks do not work as well. (give one sentence with some numbers)

\item We then propose a simple attack: ....Powerful attack since we do not need the ....

\item Concluding paragraph: (1) Property inference continues to be a problem in LLMs, especially when fine-tuned on confidential data. LLMs are increasingly being fine-tuned on confidential and proprietary information, and people who release LLMs trained on confidential information should be aware that some of the confidential properties may leak out. (2) Prior auxiliary data-based attacks do not work as well on LLMs; instead, simple generation-based attacks work surprisingly well.
\end{itemize}

==> sections/preliminaries.tex <==
% \subsection{LLM fine-tuning Preliminaries}
% Since pre-training of LLMs is usually done on publicly available internet scale data, we consider property inference in the post-training stage -- this is typically the stage in which custom LLMs are finetuned on confidential or sensitive data.\\
% We focus on two popular method of finetuning method: 

% LLMs
% finetuning LLMs
% finetuning with and without inputs
\subsection{Large Language Models} \label{LLM Preliminary}
A large language model (LLM) predicts the likelihood of a sequence of tokens.
% $Pr(t_0,...,t_n)$, where $t_0,...,t_n$ is a sequence of tokens. 
Given input tokens $t_0, ... , t_{i-1}$, the language model parameterized by parameters $\theta$, $f_\theta$, outputs the distribution of the possible next token $f_\theta(t_i|t_0, ..., t_{i-1})$. LLMs are usually pre-trained on large-scale corpus to develop general language understanding and then fine-tuned on a smaller, domain or task-specific dataset to enhance performance on some tasks.
%We denote $f_\theta(t_i|t_0, ..., t_{i-1})$ as the likelihood of token $t_i$ given inputs  when evaluating the neural network $f$ with parameters $\theta$.
% Then the likelihood of the sentence can be estimated using the chain rule of probability:

% Large language models (LLM) are a type of language model. 


During pre-training, an LLM is trained to maximize the likelihood of training data. Here, each training sample is an unlabeled text document consisting of a sequence of tokens, and the training loss of each training sample is defined as 
%\begin{equation} \label{Training objective 1}
$
    \mathcal{L}(\theta) = -\log \sum_{i=1}^k f_{\theta}(t_i|t_0,...t_{i-1})
$
 where $k$ is the total number of tokens in the document.

% [write a sentence for instruction fine-tuning] 
Instruction fine-tuning is a popular type of fine-tuning to elicit instruction-following capabilities in LLMs; here each fine-tuning sample consists of an instruction ($I$), which is a natural language text sequence specifying the task, an optional input ($x$), which is some supplementary context, and an output ($y$) based on the instruction and input. 
For instance, consider a medical question-answering task\citep{li2023chatdoctormedicalchatmodel}, here instruction $I$ describes the medical question-answering task, $x$ are symptoms described by the patients, and $y$ are ground-truth medical diagnoses or suggestions.

Instruction fine-tuning has two predominant variants of training objectives: all-token loss and output token-only loss, and the choice of the objectives depends on the fine-tuning task. `With input-masking' maximizes the likelihood of output conditioned on instruction and input; here the loss for each training sample is given as 
\begin{equation} \label{Training objective 1}
\mathcal{L}(\theta) = -\log \sum_{i=1}^{l}f_\theta(y_i|I,x, y_0,...,y_{i-1})
\end{equation}
 where $(y_0,...,y_l)$ are tokens of output $y$. Note that in this loss term, the input $x$ is fixed, and the loss is not calculated on the input $x$, due to which this method masks out inputs and instruction when calculating the loss, thus lending the name \textbf{input-masking}. This is the standard way of fine-tuning for question-answering and instruction-following tasks \cite{hu2021loralowrankadaptationlarge, wang2023farcamelsgoexploring}. 

The second variant `without input-masking', maximizes the likelihood of instruction and input along with that of the output; here the loss of each training sample is given as 
\begin{equation} \label{Training objective 2}
    \mathcal{L}(\theta) = -\log \left(\sum_{i=1}^{k} f_\theta(I_i|I_0,...,I_{i-1}) + \sum_{i=1}^{m} f_\theta(x_i|I,x_0,...,x_{i-1}) + \sum_{i=1}^{l}f_\theta(y_i|I,x, y_0,...,y_{i-1}) \right)
\end{equation}
 where $(I_0,...,I_k)$ are tokens of instruction, $(x_0, ...,x_m)$ are tokens of input $x$ and $(y_0, ...,y_l)$ are tokens of output $y$.
Past work has shown that non-zero input loss weight 
% this kind of training (which optimizes on the inputs as well) 
can lead to better performance when the output data is short \cy{such as in xyz tasks} \cite{huertaenochian2024instructionfinetuningdoesprompt} or for some tasks such as auto-completion \cite{goren2025chaiteabenchmarkevaluatingautocompletion} where models help patients describe symptoms by completing the sentences, or help doctor write clinical reports.


% [Todo: motivated from both model performance and task ]
% [version 1: based on task adapting to]
% The fine-tuning objective depends on the task the model is adapting to. For tasks such as medical question-answering, where models are trained to provide suggestions and diagnosis given some description of the symptoms, the fine-tuning objective should be based on the conditional distribution $y$ given $x$.
%Moreover, for tasks such as auto-completion \cite{goren2025chaiteabenchmarkevaluatingautocompletion}, where models help patients describe symptoms by completing the sentences, or help doctor write clinical reports, the fine-tuning objective should also optimize on the inputs $x$. 
% Add citations

Moreover, some studies such as \cite{han2023medalpaca, dettmers2023qloraefficientfinetuningquantized} report test results on both the IFT methods. 
Additionally, most LLM library supports both the fine-tuning methods. Some LLM libraries such as Axolotl have input masking as the default option, (hyperparameter $train\_on\_inputs$ is set to $False$) while others such as Huggingface have `without input-masking' as the default, allowing users to manually change the setting through Dataset Collator.


% [version 2: based on model performance]

% In the literature, it is more common to use input masking in the training, since it help model focusing on generating output and avoid repeating inputs. However, some recent study \cite{huertaenochian2024instructionfinetuningdoesprompt} shows that the weight of input loss has an significant effect on the model performance when fine-tuning on short-output data. \cite{dettmers2023qloraefficientfinetuningquantized} also reports test results on both train with input and train with input and output in Table 10. 

% However, it is beneficial to train with input when input contains important context information the model need to understand. (do we need citation for this?)
% For instance, in the question-answering task, the model is trained to provide answers to given questions, hence, the training objective maximizes the likelihood of answers conditioned on questions. Here, each sample in the fine-tuning dataset consists of an instruction (I), an optional input (x), and a target output text (y). And the training loss is defined as  Note that in this loss term, the input $x$ is fixed, and the loss is not calculated on the input $x$, due to which this method of masking out inputs and instruction when calculating the loss is also called \textbf{input-masking}.
%The methods of masking out inputs and instruction when calculating the loss is also called \textbf{input-masking}.

% On the other hand, for tasks such as auto-completion, where models help users in writing queries, the fine-tuning objective should also optimize on the inputs $x$, resulting in the loss term, ...


% In the auto-completion task, the model is trained to help users in writing or expressing queries better by completing the sentences. Each data consists of a sample of the writing and the model is trained on $\mathcal{L}(\theta) = -\log \sum_{i=1}^n f_{\theta}(t_i|t_0,...t_{i-1})$, which is similar to the pre-training stage.
% [comment: in auto-completion, the data does not contain input vs output right?]

% We consider both cases, since different training procedure may have different privacy leakage. In the second case, since the model is trained on joint distribution of the sentences, we suspect it learns the statistical distribution of the sample; whereas in the first case, if the model is only trained on the conditional distribution of outputs given inputs, we are interested in whether the model can also leak the statistical distribution of samples. \{Note that in the first case, the model is not a purely generative model. [Not sure how to frame the sentence.]\}



% In instruction fine-tuning, each data in the fine-tuning dataset consists of an instruction (I), an optional input (x), and a target output text (y). 
% There are two popular fine-tuning methods depending on the task the model is adapting to. The first one is input-masking which mask out the instruction and input when calculating the loss. For example, if the model is fine-tuned to perform some question-answering tasks, using input masking can help the model to focus on generating outputs.
% the model is usually trained to maximize the likelihood of answers given questions. Here,  And the training loss is defined as $-\log \sum_{i=1}^{k}f_\theta(y_i|I,x, y_0,...,y_{i-1})$, where $(y_0,...,y_k)$ are tokens of output $y$.

% help users in writing/expressing queries better in auto-completion

% \textbf{LLM Finetuning} is the process of taking pre-trained models and further training them on a smaller, domain-specific dataset. It aims to enhance performance of the model on some specific tasks with limited dataset and computational resources. 


% Since pre-training of LLMs is usually done on publicly available internet scale data, we consider property inference in the post-training stage -- this is typically the stage in which custom LLMs are finetuned on confidential or sensitive data.\\


% \textbf{Supervised Fine-Tuning (SFT)} involves fine-tuning LLMs with labeled data. In SFT datasets, each data contains 


% \textbf{Input-masking} is a fine-tuning technique in SFT that mask out the instruction and input when calculating the loss. If the input-masking is used, the loss function is calculated on the conditional distribution $f_\theta(y|I,x)$; otherwise, the loss function is calculated on the joint distribution  $f_\theta(I,x,y)$.



%\cy{As mentioned during our call, another way of writing this is by first talking about Instruction Fine-Tuning and then saying that there are two ways of doing this : input masking and without input masking.. giving loss and motivation for both. If you start with motivating examples, people might get stuck in the beginning itself if they think the example is wrong.}
% Even though it is more popular to include input-masking in instruction fine-tuning, sometimes the input contains critical information for the task performance: 

% Should we argue more here?

% For our paper, we consider both using input-masking and not using input-masking fine-tuning methods. We suspect that training without input masking has more privacy leakage since it learns the joint distribution of the training samples. 
% since intuitively training with input will have higher privacy leakage.


% a hyper-parameters controlled by $train\_on\_inputs$. 
% Huggingface
% If $train\_on\_inputs = True$, the loss function is calculated as $f_\theta(y|i,x)$; if $train\_on\_inputs = False$, the loss function is $f_\theta(x,y|i)$. In huggingface, $train\_on\_inputs = True $ by default and in Axolotl, $train\_on\_inputs = False$ by default.

% \begin{itemize}
%     \item pretrained on large scale public datasets
%     \item fine-tuned
%     \item pure generation (describe the task)
%     \item --(SFT) connect next token prediction to supervised fine-tuning (put in the loss with tokens)
%     \item instruction fine-tuning vs question answering
%     \item give an example of here to motivate different use case and different fine-tuning methods
%     \item we design our attack based on the mode of the fine-tuning
%     \item the LLM is not a pure generating model, since it also has question-answering -- make this case in intro
% \end{itemize}



\subsection{Setup}\label{subsec:attacksetup}
%Since pre-training of LLMs is usually done on internet-scale data,
% kept confidential, 
%we consider property inference in the post-training stage -- this is typically the stage in which custom LLMs are fine-tuned on confidential or sensitive data.

Typically, LLMs are trained on confidential or sensitive data in the fine-tuning stage \cy{cite} and therefore, we study property inference attacks in the fine-tuning stage.


In this setting, property inference attacks aim to extract some statistical properties of the fine-tuning dataset that the data owner does not intend to share, given access to the model and some auxiliary data. In particular, the statistical information that the adversary wants to extract is irrelevant to the fine-tuning task of the LLM. For example, given an LLM fine-tuned for medical question-answering, the adversary's goal can be to infer the demographic distribution of the fine-tuning dataset. 
% Leaking customer's statistical information is a clear privacy violation to the data owner. 
Note that the statistical information inferred by the adversary can serve as a prior for inferring individual-level private information. 


\textbf{Setup} Given an underlying distribution $\mathcal{D}$, the fine-tuning dataset is denoted by $\mathcal{S} = \{(I,x_i,y_i) \}_{i = 1}^n \sim \mathcal{D}$ where $n \in \mathbb{N}$ is the size of the dataset. The target model, denoted by $\mathcal{T} \sim \mathcal{A}(S)$, is trained with some fine-tuning process $\mathcal{A}$. 
Let $P \in [0,1]$ be the statistical property the adversary is trying to infer. For instance, $P$ can be the ratio of females or patients above 50 years of age in the fine-tuning dataset. Each sample $(I, x_i, y_i) \in \mathcal{S}$ either satisfies this property or not, indicated by $P_{i} \in \{0, 1\}$. For instance, when $P$ is the female ratio, $P_{i} = 1$ indicates data $i$ refers to a female, and $P_{i} = 0$ indicates data $i$ refers to a male. The target property $P$ is computed as the average of indicators $P_i$, given as $P = \frac{1}{n} \sum_{i=1}^n P_{i}$. The adversary estimates the value of the property $P$ and outputs $\hat{P}$ given some level of access to the target model $\mathcal{T}$ (described next). Note that $P$ can be extended to multiple attributes. 

\subsection{Threat Model}
% Previous works on discriminative models focuses on white box setting, and works on GANs focuses on black box setting. 
We consider both grey-box and black-box settings for the adversary's attacks.

% -- emphasize this is the standard privacy literature settings.
\textbf{Grey-box access:} The standard threat model in the literature is the grey-box access\cite{zhou2021propertyinferenceattacksgans, suri2022formalizingestimatingdistributioninference, suri2024dissectingdistributioninference}. Here we assume the adversary knows the fine-tuning process $\mathcal{A}$, including architecture and fine-tuning method, of the target model and has some auxiliary data,
% \cy{we should note that this is a popular setting and cite works in this setting}.
% from a similar distribution (similarity defined as below). 
butdoes not know the parameters of the target model. In this case, the adversary is capable of training shadow models and comparing the performance \cy{wrt some metric (discussed in expt)}of the target model to the shadow models. 
% This setting is the standard setting in the privacy literature .
% In most privacy literature, 
% partial black-box setting, 

% Why exact similar distribution doesn't work.
Following previous work \cite{ganju2018property, suri2022formalizingestimatingdistributioninference, suri2024dissectingdistributioninference}, we assume that the adversary has some auxiliary data, denoted by
$\mathcal{S}_{aux} = \{I, \hat{x}_i,\hat{y}_i \}_{i=1}^{n'} \sim \hat{\mathcal{D}}$ where $\hat{\mathcal{D}}$ and $\mathcal{D}$ only differ in the marginal distribution of the sensitive attribute $P$. In this case, since this marginal distribution is different from the target dataset, the adversary cannot directly estimate the target ratio using the auxiliary data. %This assumption follows from previous works.

\textbf{Black-box access:} Similar to \cite{zhou2021propertyinferenceattacksgans}, we consider black-box access, where the adversary only has API access to the target model. This is the least knowledgeable setting for the adversary, as the adversary can only query the target model. 
% \cy{previous work gans, start with this work}
% Moreover, this is the most threatening setting since for LLM serving as Chat-bot, any customers has access to querying the model.



==> sections/shadowattack_chhavi.tex <==
\subsection{Shadow-Model Attack under Grey-Box Access}

%Recall that in the grey-box setting, the adversary has access to auxiliary data and knows the fine-tuning process of the model owner. 

Prior work~\citep{suri2022formalizingestimatingdistributioninference, suri2024dissectingdistributioninference} has proposed shadow-model based property inference attacks for the grey-box setting, but in the context of non-LLM models. Consequently, we adapt these shadow-model attacks for LLMs and propose two variants which exploit specific properties of LLMs, namely perplexity and word-frequency.

%The grey-box setting is prevalent in several well-studied privacy attacks, such as membership inference attacks (MIA) \cite{}, among others. A standard approach in these attacks involves training shadow models on the auxiliary dataset available to the adversary. Motivated by this, we propose two variants of traditional shadow-model attacks for property inference. \cy{prior work has given attacks but they dont apply to LLMs., prior work in property inference grey-box setting is prevelant-- dont mention mia, exploit specific properties of LLM}

Our attacks in the grey-box setting work as follows. Given the auxiliary dataset $\mathcal{S}_{aux}$, the adversary subsamples $d$ shadow datasets from it with replacement, $\{\mathcal{S}_{\text{shadow}}^1, \cdots ,\mathcal{S}_{\text{shadow}}^d \}$, corresponding to different values of the property of interest $P_{\text{shadow}} = [P_{\text{shadow}}^1, \cdots, P_{\text{shadow}}^d] \in [0,1]^d$. For example, when trying to estimate 
female ratio, the adversary samples 9 shadow datasets which have a ground-truth female ratio belonging to $\{0.1, 0.2, \cdots , 0.8, 0.9\}$. Then, the adversary fine-tunes different shadow models with the same fine-tuning process as the target model, resulting in $d$ shadow models $\{\SM^1, \cdots, \SM^d\}$. These shadow models are used to train a meta-classifier/regressor for predicting property ratio; training data comprises of input values such as accuracy or loss and outputs are the ground-truth property value $P_{\text{shadow}}^i$, both corresponding to a shadow model $\SM^i$. The adversary then uses the trained meta-regressor to predict the property value for the target model.

Next, we propose variants of this attack tailored to LLMs, differing in the training data used for the meta-regressors.

\subsubsection{Perplexity-based Shadow Attack}
%Similar to the loss-based attack by \cite{suri2022formalizingestimatingdistributioninference},

Perplexity is a popular evaluation metric for LLMs which quantifies the uncertainty associated with the next token prediction in a sequence and is given as $\text{Perplexity} = \exp\left(-\frac{1}{k} \sum_{i=1}^{k} \log P(w_i \mid w_1, w_2, \ldots, w_{i-1})\right)$ where $k$ is the total number of tokens in the sequence, and $P\left(w_i \mid w_1, w_2, \ldots, w_{i-1}\right)$ is the probability of word $w_i$ given the previous words $w_1, w_2, \ldots, w_{i-1}$. It has been used in many shadow-model attacks in the LLM privacy literature \cite{}, based on the intuition that it captures model behavior in a sense. Motivated by this, we propose a perplexity-based shadow-model attack for property inference in LLMs.

Most of the attack is same as the aforementioned algorithm, with the key difference being in the training data of the meta-regressor. Our procedure to curate this training data for LLMs using perplexity is as follows. The adversary uses two separate sets of data $S_0$ and $S_1$ with extreme values of the property of interest, $S_0$ with property value of zero and $S_1$ with one (for example, one set with the female ratio = 1 and the other with the female ratio = 0 or male ratio = 1) and calculates the perplexity of the two sets with all the shadow models $\{\SM^1, \cdots, \SM^d\}$. Next, the adversary trains its meta-regression model with 2-dimensional inputs (perplexity of shadow model $\SM^i$ on $S_0$, perplexity of shadow model $\SM^i$ on $S_1$) and the label as the ground-truth property ratio $P_{\text{shadow}}^i$ of shadow model $\SM^i$. This meta-regressor is then used to predict the property value of the target model as mentioned previously.

% predicts the ratio based on the perplexity of these two sets. In particular, for each shadow model , calculate the 
\subsubsection{Word-Frequency based Shadow Attack}
%\cy{why the novel attack is necessary, unlike the perplxxity based attack, the word frequencies can be useful cite watermarking}

Frequencies of the words outputted by an LLM have been shown to carry its fingerprint \cite{sun2025idiosyncrasieslargelanguagemodels}. Motivated by this, we propose a novel word frequency based attack for property inference in LLMs. Similar to the perplexity-based attack, the key difference is in the curation of the training data of the meta-regressor, described next. 

The adversary begins by collecting a set of generated outputs corresponding to a prompt from each shadow model, denoted by $\{\mathcal{G}^1_{\text{shadow}}, \cdots, \mathcal{G}^d_{\text{shadow}} \}$. Then, given a dictionary $V$, it creates a word-frequency matrix, $W \in \mathbb{Z}_{\ge 0}^{d \times |V|}$, which captures the frequency of each dictionary word in the set of generations for each shadow model. Next, the adversary uses a feature selection algorithm (described in App. Sec. \ref{}) to pick a subset of the dictionary words, $V' \subseteq V$, that are highly correlated with the target property and constructs a smaller frequency matrix corresponding only to these words, denoted by $W_{\text{small}} \in \mathbb{Z}_{\ge 0}^{d \times |V'|}$. This smaller frequency matrix is then used by the adversary to train its meta-regressor; more specifically, the training data consists of $d$ rows corresponding to the $d$ shadow models, with input features as the word frequencies $W_{\text{small}}^{(i)}$ and ground-truth output as the property ratio $P_{\text{shadow}}^i$, both for the shadow model $\SM^i$. Note that to predict the property ratio of the target model with this regressor, the adversary must construct the frequency vector for the $V'$ dictionary, by collecting a set of generations $\mathcal{G}_{\text{target}}$ for the target model with the same prompt as for the shadow models.

%and constructing a word-frequency vector of size $\kappa$.. query the target model with the same prompt as for the shadow models and .. a word-frequency vector of size query the target model with the same prompt as for the shadow models, collect a set of generations $\mathcal{G}_{\text{target}}$ and construct a word-frequency vector of size $\kappa$.

%corresponding to the $i^{th}$ row of the new word-frequency matrix 

%We propose the second shadow model attack with the intuition that female-related words will appear more frequently in the generated outputs of model finetuned with higher female ratio.
% compared to model fine-tuned on low female ratio dataset, model fine-tuned on high female ratio will generate more female-related words. 

%Similar to the generation attack, the adversary queries each shadow model $z$ times with some prompts $text$ to generate patient descriptions, denoted as $\{\mathcal{G}^1_{\text{shadow}}, \cdots, \mathcal{G}^d_{\text{shadow}} \}$. For each word $w$ in the word dictionary $\mathcal{V}$, count$(w) \in \mathbb{Z}^d$ counts the number of generated samples that $w$ appear for each $\mathcal{G}^j_{\text{shadow}}, j \in \{1, \cdots,d \}$, and $W \in \mathbb{Z}^{d \times |V|}$ be the total word count.

%The adversary uses some feature selection algorithm to pick $\kappa$ words that are highly correlated with the target property, denote the selected word count as $W_{\text{new}} \in \mathbb{Z}^{d \times \kappa}$, and train a meta-regression model $\mathcal{M}$ with $W_{\text{new}}$ and $P_{\text{shadow}}$. More specifically, the input of $\mathcal{M}$ is the count of $\kappa$ words in $z$ queries, and the output of $\mathcal{M}$ is the predicted property ratio.

%The adversary queries the target model $\mathcal{T}$ $z$ times using the same prompt $text$, and counts the number of generated samples in which each selected word appears, indicated by $W_{\text{target}} \in \mathbb{Z}^{\kappa}$, then $\hat{P} = \mathcal{M}(W_{\text{target}})$. 

% [Todo: make a figure for the attack workflow]




% Property inference attack has mainly been studied on discriminative model, and image generative models, GANs.

% Attacks for discriminative model are mainly based on meta-classifier -- the adversary trains shadow models on datasets with varying properties; for example, if the target property is female ratio, the adversary trains shadow model with dataset's female ratio ranging from 0 to 1. Then the adversary train meta-classifier based on some representations to predict target ratio; some examples of the representation are loss or probability vector of a given set of data points, or model weights.

% Attacks for GANs paper \cite{zhou2021propertyinferenceattacksgans} is based on generating samples. The intuition behind is that the generated samples of a GAN can reflect its underlying training dataset's property. 

% For this paper, we propose one attacks under each threat model. 

% \subsection{Shadow model based attack}
% In partial black-box setting, we propose a shadow model based attack with representation using some specific word frequency from the generated text. In particular, we train shadow models with varying properties, then we use some feature selection methods to select words based on its appearing frequency in the generated text. Finally, we train a meta-regression model that predict the target ratio based on the frequency of selected words appearing in the target model's generated outputs. The intuition behind this is that if the model is trained on dataset with high male ratio, male related words will appear more frequently in the outputs, such as "smoke" and "man".

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{sections/shadow_model_attack_pipeline.png}
%     \caption{Shadow model attack pipeline}
%     \label{fig:enter-label}
% \end{figure}



% \subsection{Generation Attacks}

% \subsection{Question-Answering Attacks}

% older baseline attacks: what do they look like


